Model-free Reinforcement Learning for Stochastic Stackelberg Security Games

In this paper, we consider a sequential stochastic Stackelberg game with two players, a leader and a follower. The follower has access to the state of the system while the leader does not. Assuming that the players act in their respective best interests, the follower's strategy is to play the best response to the leader's strategy. In such a scenario, the leader has the advantage of committing to a policy which maximizes its own returns given the knowledge that the follower is going to play the best response to its policy. Thus, both players converge to a pair of policies that form the Stackelberg equilibrium of the game. Recently,~[1] provided a sequential decomposition algorithm to compute the Stackelberg equilibrium for such games which allow for the computation of Markovian equilibrium policies in linear time as opposed to double exponential, as before. In this paper, we extend the idea to an MDP whose dynamics are not known to the players, to propose an RL algorithm based on Expected Sarsa that learns the Stackelberg equilibrium policy by simulating a model of the MDP. We use particle filters to estimate the belief update for a common agent which computes the optimal policy based on the information which is common to both the players. We present a security game example to illustrate the policy learned by our algorithm. by simulating a model of the MDP. We use particle filters to estimate the belief update for a common agent which computes the optimal policy based on the information which is common to both the players. We present a security game example to illustrate the policy learned by our algorithm.

==> STACKELBERG/0Config.tex <==
\usepackage{bbm}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{mathrsfs}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage[english]{babel}
% \usepackage{amsthm}
\usepackage{epstopdf}
\usepackage{textcomp}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}

\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{lemma*}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}




\renewcommand{\hat}{\widehat}
\renewcommand{\bar}{\overline}

\newcommand{\cN}{\mathcal{N}}
\newcommand{\cT}{\mathcal{T}}



\newcommand{\ux}{\underline{x}}

\newcommand{\uF}{F}
\newcommand{\nn}{\nonumber}    
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\defeq}{\buildrel\triangle\over =}
\newcommand{\sq}[1]{\left[#1\right]}
\newcommand{\cm}[1]{\left(#1\right)}
\newcommand{\bm}[1]{\left\{#1\right\}}
\newcommand{\review}[1]{\textcolor{red}{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}

\newcommand{\mP}{\mathbb{P}}
\newcommand{\mE}{\mathbb{E}}
\newcommand{\mR}{\mathbb{R}}

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cKg}{{\mathcal{K}}^{\tilde{\gamma}}}

\newcommand{\tgamma}{\tilde{\gamma}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\ttheta}{\tilde{\theta}}


\newcommand{\pih}{\hat{\pi}}
\newcommand{\muh}{\hat{\mu}}
\newcommand{\pit}{\tilde{\pi}}
\newcommand{\gammah}{\hat{\gamma}}
\newcommand{\Fh}{\hat{F}}

% Follower
\newcommand{\sigf}{\sigma^f}
\newcommand{\tsigf}{\tilde{\sigma}^f}
\newcommand{\siglf}{{\sigma^l,\sigma^f}}
\newcommand{\tgammatf}{{\tilde{\gamma}_t}^f}

% Leader
\newcommand{\tgammatl}{{\tilde{\gamma}_t}^l}


==> STACKELBERG/0Glossary.tex <==
\usepackage{xspace}
\usepackage[acronym,nogroupskip,nonumberlist,nopostdot]{glossaries}
\glsdisablehyper

% WIRELESS AND DIGITAL COMMS
\newacronym{mdp}{MDP}{Markov decision process}
\newacronym{ne}{NE}{Nash equillibrium}
\newacronym{mfe}{MFE}{mean-field equillibrium}
\newacronym{mpe}{MPE}{Markov perfect equillibrium}
\newacronym{mfg}{MFG}{mean-field game}
\newacronym{rl}{RL}{reinforcement learning}
\newacronym{marl}{MARL}{multi-agent reinforcement learning}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{ssg}{SSG}{Stackelberg security game}
\newacronym{pse}{PSE}{perfect Stackelberg equilibrium}
\newacronym{mpse}{MPSE}{Markov \gls{pse}}
\newacronym{pomdp}{POMDP}{partially observed \gls{mdp}}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{pbe}{PBE}{perfect Bayesian equilibrium}
\newacronym{gmfg}{GMFG}{graphon mean-field game}
\newacronym{gmfe}{GMFE}{graphon mean-field equillibrium}
\newacronym{spe}{SPE}{sub-game perfect equillibrium}
\newacronym{mkv}{MKV}{McKean-Vlasov}

\newcommand{\mdp}{\gls{mdp}\xspace}
\newcommand{\gne}{\gls{ne}\xspace}
\newcommand{\mfe}{\gls{mfe}\xspace}
\newcommand{\mpe}{\gls{mpe}\xspace}
\newcommand{\mfg}{\gls{mfg}\xspace}
\newcommand{\mfgs}{\glspl{mfg}\xspace}
\newcommand{\rl}{\gls{rl}\xspace}
\newcommand{\marl}{\gls{marl}\xspace}
\newcommand{\ssg}{\gls{ssg}\xspace}
\newcommand{\ssgs}{\glspl{ssg}\xspace}
\newcommand{\pse}{\gls{pse}\xspace}
\newcommand{\mpse}{\gls{mpse}\xspace}
\newcommand{\pomdp}{\gls{pomdp}\xspace}
\newcommand{\pbe}{\gls{pbe}\xspace}
\newcommand{\gmfg}{\gls{gmfg}\xspace}
\newcommand{\gmfe}{\gls{gmfe}\xspace}
\newcommand{\spe}{\gls{spe}\xspace}
\newcommand{\spes}{\glspl{spe}\xspace}
\newcommand{\mkv}{\gls{mkv}\xspace}

==> STACKELBERG/1Introduction.tex <==
% Introduction and explanation and use of RL
Stackelberg games are a very useful tool to model strategic interactions where there is a dominant player called the leader who commits to a policy and a follower that \emph{observes} the leader's policy and plays its best response to it. With the knowledge that the follower will play the best response, the leader can devise an optimum strategy that maximizes its own rewards. Such games, also termed as Stackelberg security games, have become very popular in the recent decade in building and analyzing real world security systems in areas such as airports, seaports, and wildlife parks~\cite{fang2015security}. In such games, the leader has an inherent advantage that enables it to commit to a strategy that benefits it irrespective of the strategy followed by the follower given that it is rational and will play the best response. Such one shot equilibrium games have also proven useful for economic firms to analyze markets and take competitive risks.

Most of the prior work consider single shot Bayesian game models where the leader and the follower interact only once. However, most practical systems entail a periodic interaction between the leader and the follower. Computing Stackelberg equilibria for such stochastic games was unknown. Recently~\cite{Vasal} presented a sequential decomposition algorithm to compute \mpse of such games. Solving a dynamic stochastic Stackelberg game when the follower has a private Markovian state is computationally challenging. This is because, unlike other games, dynamic games of asymmetric information have players' strategies that are coupled across time. Since strategy of a player is a mapping from each history of the game which grows exponentially with time, the space of strategies of the players is double exponential, rendering such problems intractable. Recently, there has been results on sequential decomposition of certain classes of games of asymmetric information~(\cite{Vasal2016,Vasal2017,Vasal}). In repeated Stackelberg security games, there have been other approaches to mitigate this issue. For instance,~\cite{Kar2015} considers a repeated Stackelberg game and uses a new human behavior model to study such games. \cite{Balcan2015} consider a learning theoretic approach to study a repeated Stackelberg game between attacker and defender where they use regret analysis to learn attacker types, and show sub-linear regret for both complete and partial information models. There also have been efforts to develop \rl algorithms to study models with asymmetric information in~\cite{Kononen2003} for repeated Bayesian Stackelberg games.

Kalman filters have been widely used for Gaussian state space modelling but the advent of sequential monte carlo methods can be attributed to certain applications where non-Gaussian state space modelling was required~\cite{kitagawa1996monte}. Particle filters are sequential monte carlo filters that approximate the belief on a state, in other words, the probability of a system of being in a particular state, from an empirical distribution based on the observed history when model dynamics are unknown~\cite{Douc2005,Crisan2002}. It is widely popular in applications like robotics for localizations and fault dynamics, where most of the times the environment is non-Gaussian and needs to learned based on collected samples and observations~\cite{rekleitis2004particle}. These methods utilize a $K$ number of random samples or \emph{particles}, where $K$ is large, to represent the posterior probability of the state based on the observations.


% Our Contribution
In this paper, we propose an \rl algorithm with particle filters to learn the Stackelberg equilibrium strategies for a rational, leader and follower, when the players are unaware of the dynamics of the game. The algorithm learns the $Q$ values using the Expected Sarsa and then solves a fixed point equation for the follower and a maximization equation for the leader to converge upon the strategies. We use a common agent approach~\cite{Nayyar2013a} wherein a fictitious common agent has access to the common information that is shared between the players and uses it to compute a belief on the private state. It then solves for the optimal policies using the \rl algorithm and updates the belief using the particle filters. The use of \rl algorithm with particle filters for solving for Stackelberg equilibrium is novel. We illustrate our algorithm by determining the strategies for a realistic security game example to show that the algorithm derived, coincides with the optimal strategy that was obtained in~\cite{Vasal}, where it was assumed that the dynamics of the game were known.

% Paper Flow
The paper is structured as follows. The model is presented in Section~\ref{sec:Model} followed by a discussion on the sequential decomposition algorithm in Section~\ref{sec:Preliminaries}. We present our proposed algorithm in Section~\ref{sec:Algorithm} and prove convergence to the Stackelberg equilibrium in Section~\ref{sec:Conclusion}. In Section~\ref{sec:Example}, we provide an example to showcase our results and conclude in Section~\ref{sec:Conclusion}.

\subsection{Notation}

We use uppercase letters for random variables and lowercase for their realizations. For any variable, subscripts represent time indices and superscripts represent player identities, `$l$' for the leader and `$f$' for the follower. For any finite set $\mathcal{S}$, $\mathcal{P}(\mathcal{S})$ represents space of probability measures on $\mathcal{S}$ and $|\mathcal{S}|$ represents its cardinality. We denote by $P^{\sigma}$ (or $E^{\sigma}$) the probability measure generated by (or expectation with respect to) strategy profile $\sigma$ and the space for all such strategies as $\mathcal{K}^\sigma$. We denote the set of real numbers by $\mathbb{R}$. All equalities and inequalities involving random variables are to be interpreted in an \emph{a.s.} sense. 

==> STACKELBERG/2Model.tex <==

Consider a stochastic Stackelberg game over a time horizon $\cT$ with perfect recall between two players: a leader and a follower. The actions and the states are defined over finite sets $\cA$ and $\cX $ respectively. $\cA^l$ denotes the action set of the leader while $\cA^f$ represents that of the follower. The state $x_t$ evolves as the following controlled Markov process
\begin{align}
	\cP\left(x_t|a_{1:t-1},x_{1:t-1}\right) &=  \tau\left(x_t|a_{t-1},x_{t-1}\right), 
\end{align}
where $a_t = \cm{a_t^l,a_t^f}$ are the actions of the leader and the follower. The action history $a_{1:t-1}$ is shared between both the players as common information. However, only the follower has access to the private information $x_{1:t}$. The leader observes the common information $a_{1:t-1}$ and takes action $a_t^l\in \cA^l$ while the follower observes the private information $x_{1:t}$ and the common information $a_{1:t-1}$ and takes action $a_t^f\in \cA^f$. 


% Let $ \sigma \defeq(\sigma^i)_{i\in \{l,f\}}$ be a strategy profile of both the players where $\sigma^i = ( \sigma^i_t)_{t \in\cT}$ represents the probabilistic strategy of player $i\in\{l,f\}$ with $\sigma^l_t : \cA^{t-1} \to \mathcal{P}(\cA^l)$ and $\sigma^f_t : \cA^{t-1}\times\cX^t \to \mathcal{P}(\cA^f)$ respectively for leader and follower. At the end of interval $t$, the leader receives an instantaneous reward $R_t^l(x_t,a_t)$ and the follower receives an instantaneous reward $R_t^f(x_t,a_t)$ and the players discount their rewards by a discount factor $\delta\leq 1$. The goal of the players is to maximize their expected sum of discounted returns given as 
% \begin{align}
% 	\label{Eqn:j_func1}
% 	J^{f,\sigma^f,\sigma^l}_t=\mathbb{E}^{\sigma^f_{t:T}, \sigma_{t:T}^l}\left[\sum_{k=t}^{T}\delta^{k-t}R_t^f\left(X_k,A_k\right)\vert x_{1:t},a_{1:t-1}\right],
% \end{align}
% \begin{align}
% 	\label{Eqn:j_func2}
% 	J^{l,\sigma^f,\sigma^l}_t=\mathbb{E}^{\sigma^l_{t:T},\sigma_{t:T}^f}\left[\sum_{k=t}^{T}\delta^{k-t}R_t^l\left(X_k,A_k\right)\vert a_{1:t-1}\right].
% \end{align}

==> STACKELBERG/3Preliminaries.tex <==

In this section, we discuss the sequential decomposition algorithm which used to compute the Stackelberg equilibrium policies for the case when the model is known to the players.

\subsection{Stackelberg Equilibrium}
Given a strategy profile $\sigma^l$ for the leader, the follower maximizes its own total discounted expected rewards over a finite horizon $T$ as
\begin{align}
	\max_\sigf\mE^\siglf \sq{\sum_{t=1}^T \delta^{t-1}R_t^f\left(X_t,A_t\right)}.
\end{align}
Now, if we denote $\Lambda^f(\sigma^l)$ to be the set of all optimizing strategies for the follower, given a strategy $\sigma^l$ of the leader, we get
\begin{align}
	\Lambda^f(\sigma^l) = \arg\max_{\sigma^f} \mE^{\sigma^l,\sigma^f} \left[ \sum_{t=1}^T\delta^{t-1} R_t^f\left(X_t,A_t\right) \right].
\end{align}
With the information that follower is going to play the best response to its strategy, the leader tries to maximize its own total expected discounted rewards by finding an optimal strategy. In other words, knowing the follower's counter strategy to be $\Lambda^f(\sigma^l)$, the leader tries to solve the following maximization equation to compute its own strategy:
\begin{align}
\label{eq:Stck_eq}
	\tsigma^l \in\max_{ \sigma^l} \mE^{\sigma^l,\Lambda^f(\sigma^l)} \left\{ \sum_{t=1}^T\delta^{t-1} R_t^l(X_t,A_t) \right\}.
\end{align}
Both leader and follower successively play this game and converge upon a pair of strategies $(\tsigma^l,\tsigma^f)$ constituting a Stackelberg equilibrium where $\tsigma^f \in \Lambda^f\left(\tsigma^l\right)$.

\subsection{Perfect Stackelberg equilibrium}
\label{sec:PBSE}

The notion of \pse, as introduced in~\cite{Vasal2019a}, is in line with the \pbe discussed in~\cite{Fudenberg1991}. In the context of the game, the leader and the follower play their actions $a_t^l\sim \tsigma^l_t\left(\cdot|a_{1:t-1}\right)$ and $a_t^f\sim \tsigma^f_t(\cdot|a_{1:t-1},x_t)$ with $\tsigma = \left(\tsigma^f,\tsigma^l\right)$ constituting the Stackelberg equilibrium.

Assume $(\tsigma,\mu)$ is a \pse of the game, where $\mu = (\mu_t)_{t\in[T]}$ and $\tsigma = \left(\tsigma^f,\tsigma^l\right)$ with $\tsigma^f \in \Lambda_t^f(\tsigma^l)\ \forall \ t\in[T]$. For any $t$ and action history $a_{1:t-1}$, $\mu_t[a_{1:t-1}]\in\cP(\cX)$ is the equilibrium belief on the current follower's state $x_t$, i.e. $\mu_t[a_{1:t-1}](x_t)=\mP^{\tsigma}(x_t|a_{1:t-1})$. For any given $\sigma^l$, $\Lambda_t^f(\sigma^l)$ be defined as~$\forall h_t^f$,
\begin{align}
 	\label{Eqn:BRf}
 	\Lambda_t^f(\sigma^l) \defeq \arg\max_{\sigma^f} \mE^{\sigma^l,\sigma^f,\mu_t} \left[ \sum_{n=t}^T \delta^{n-t}R_n^l(X_n,A_n) |h_t^f\right]
 \end{align}
and
\begin{align}
	\label{Eqn:sigmaL}
 	\tsigma^l \in\max_{ \sigma^l} \mE^{\sigma^l,\Lambda^f(\sigma^l),\mu_t} \left[ \sum_{n=t}^T \delta^{n-t}R_n^l(X_n,A_n) |h_t^c\right].
\end{align}
where $h_t^f =(a_{1:t-1},x_{1:t})$ and $h_t^c = a_{1:t-1}$.

For the case of \pse the sum of expected returns can be expressed as 
\begin{align}
	\label{Eqn:j_func1}
	&J^{f,\sigma^f,\sigma^l,\pi}_t=\nn\\
	&\mathbb{E}^{\sigma^f_{t:T}, \sigma_{t:T}^l,\pi_t}\left[\sum_{k=t}^{T}\delta^{k-t}R_t^f\left(X_k,A_k\right)\vert x_{1:t},a_{1:t-1}\right],
\end{align}
\begin{align}
	\label{Eqn:j_func2}
	J^{l,\sigma^f,\sigma^l,\pi}_t=\mathbb{E}^{\sigma^l_{t:T},\sigma_{t:T}^f,\pi_t}\left[\sum_{k=t}^{T}\delta^{k-t}R_t^l\left(X_k,A_k\right)\vert a_{1:t-1}\right].
\end{align}


\subsection{Common agent approach}

We use the common agent approach in line with the common information approach that was used in~\cite{Nayyar2013a}. An arbitrary common agent with access to the common information $a_{1:t-1}$ generates prescription functions $\gamma_t = (\gamma_t^l,\gamma_t^f)$. The prescription functions $\gamma_t^l\in \cP(\cA^i)$ and $\gamma_t^f:\cX^t\to  \cP(\cA^i)$ are used by the leader and the follower to generate their actions as $a_t^l \sim\gamma_t^l(\cdot)$ and $a_t^f \sim\gamma_t^f(\cdot|x_{1:t})$. 

We denote the prescription functions as $\gamma_t = (\gamma_t^l,\gamma_t^f)$ as $\theta_t[\pi_t]$ with $\pi_t(x_t) = P^{\theta}(x_t|a_{1:t-1})$. In other words, the Markovian common agent computes the prescription functions as function of the belief state $\pi_t$, which it derives from the common information $a_{1:t-1}$. The belief state $\pi_t$ is given as
\begin{align}
	\pi_t = \mP^{\ttheta}\cm{x_t\vert a_{1:t}}
\end{align}
which denotes the distribution of the state conditioned on the observed action history. The follower uses $\gamma_t^f$ to operates on its current private state $x_t$ to produce its action $a_t^f$, i.e. $\gamma_t^f : \cX\to \cP(\cA^f)$ and $a_t^f \sim\gamma_t^f(\cdot|x_t)$. while the leader uses $\gamma_t^l$ to produce its action $a_t^l$ as $\gamma_t^l \in \cP(\cA^f)$ and $a_t^l \sim\gamma_t^f(\cdot)$.

In order to track the belief state $\pi_t$ we derive a recursive equation given a policy $\ttheta_t$. 

\begin{lemma} For any given policy of type $\theta$, there exists update functions $F$, independent of $\theta$, such that
\label{Lemma:belief_state}
	\begin{align}
	\label{eq:F_update}
		\pi_{t+1} = F(\pi_t,\gamma_t^f,a_t) 
	\end{align}
\end{lemma}
which can be elaborated using the Bayes' theorem as
\begin{align}
\label{Eqn:pit_recursive}
	\pi_{t+1}\left(x_{t+1}\right) &= \mP^\theta\left(x_{t+1}\vert a_{1:t}\right)\nonumber\\
								  &=\frac{\sum_{x_t\in\cX}\pi_t\left(x_t\right)\gamma_t^f\left(a_t^f\vert x_t\right)Q_x\left(x_{t+1}\vert x_t, a_t\right)}{\sum_{x_t\in\cX}\pi_t\left(x_t\right)\gamma_t^f\left(a_t^f\vert x_t\right)}
\end{align}

In summary, at time $t$, the common agent observes the action history $a_{t-1}$ and generates the optimal policy $\ttheta$ as a function of the belief $\pi_t$. Corresponding to each belief $\pi_t\in\Pi$, the generated prescription function $\tgamma_t=\cm{\tgamma_t^f,\tgamma_t^l}$ specifies the actions to be taken by the players. The optimal policy and the actions thus generated are used to obtain the next belief $\pi_{t+1}$ using~\eqref{Eqn:pit_recursive}. 

\subsection{Particle Filters}
\label{sec:particle_filter}
The main challenge in computing the updated belief $\pi_{t+1}$ from current belief $\pi_t$ without knowledge of the transition function $\tau$.  Particle filters are sequential monte carlo filters that approximate the state distribution from an empirical distribution based on the observed history. These methods utilize a $K$ number of random particles to represent the posterior probability of the state based on the observations.

These filters approximates the belief state $\pi_t$ by a set of $K$ sampled points from the state space $x_t\in\cX$, updated in a sequential manner at every observation point $a_t$, which also serves as an action in our case, through a selection procedure to establish the truthfulness of the belief based on the observation. In other words, the belief using a particle filter could be expressed as,
  \begin{align}
    \pih_t=\frac{1}{K}\sum_{i=1}^Kf\cm{x_t}.
  \end{align}
  The generic particle filter called the bootstrap filter that samples the states from a previous distribution and the resamples based on observations. It is estimated using an empirical distribution given as 
  \begin{align}
    \pih^{i}\cm{x_t} \defeq \sum_{j=1}^K\delta_{x_t}w_t^j,
  \end{align}
  where $\delta_{x_t}$ is a dirac delta function made up of $K$ particles $x_t^{1:K}$. The algorithm recursively consists of two steps, a transition step to sample $K$ particles from the current distribution and to obtain the samples corresponding to the next states for each of the sample according to the transition function. This is followed by a selection step where it is resampled according to the weights $w_t$ generated based on the observations. The algorithm can be summarized as below~\cite{Coquelin,Doshi2009,Elvira2017}.

  \begin{enumerate}
    \item Initialize, $t = 0$, $x_0^i\sim\pi_t\cm{\cdot}$, set $t=1$,
    \item For $t = 1,2,3,\ldots$,\newline 
    \textbf{Importance sampling:}
    \begin{enumerate}
      \item For $ i =1 \ldots K$, sample from the model, $\hat{x}_i\sim\mP\cm{x_{t+1}\vert x_t,a_t}$
      \item For $ i = 1\ldots K$, compute the weights in proportion to the chances of the next state with the current observation $a_t$
      \begin{align}
        w_t^i=\frac{\mP^\theta\cm{a_t,\hat{x}_i}}{\sum_{j=1}^K\mP^\theta\cm{a_t,\hat{x}_j}}
      \end{align}
    \end{enumerate}
    \textbf{Selection/ resampling}
    \begin{enumerate}
      \item Resample from the list $\cm{\hat{x}_{t+1}}$ with replacement according to the weights to get $\cm{x_{t+1}}$. This is done by choosing from indices $\bm{1\ldots K}$ according to the multinomial distribution $\cm{w_1\ldots w_K}$.
      \item The new belief state estimate is then,
      \begin{align}
        \pih\cm{x_t} \defeq \sum_{i=1}^K\delta_{x_{t+1}}
      \end{align}
    \end{enumerate}
  \end{enumerate}
  
  The multinomial distribution used for resampling is one of the simplest methods that was introduced in~\cite{Vapnik1999}. This methods redistributes the samples based on their corresponding weights. Other versions of the resampling method include the stratified sampling method that reduces variance~\cite{kitagawa1996monte,Douc2005}.

  The common agent employs a $2$ parallel particle filters that estimate $\mP^\theta\cm{x_{t+1}\vert a_{1:T}}$ for each of the player given the policy $\theta$. The particle filter as a module takes in the current belief vector, the corresponding policy and the observation vector. It uses the model to sample the next steps and then computes the posterior distribution.


\subsection{Algorithm for \mpse computation}
\label{sec:Result}

In this section, we discuss the sequential decomposition algorithm stated in~\cite{Vasal2019a} but using the belief estimated using the particle filters to compute the equilibrium strategies by solving equations~\eqref{Eqn:BRf} and~\eqref{Eqn:sigmaL}.
 
\subsubsection{Backward Recursion}


In a general \rl setting, with finite state space $\cX$ and finite action space $\cA$, we can express the $Q$-value for the state action pair $\left(x_t, a_t\right)$ for all $x_t\in\cX$, $a_t\in\cA$ in terms of the reward $R_t\left(x_t, a_t\right)$ as
\begin{align}
\label{Eqn:Bellman_optimality}
	Q_t\left(x_t, a_t\right)=R_t\left(x_t, a_t\right)+\delta\mE^\tau\left[V_{t+1}\left(X_{t+1}\right)\right]. 
\end{align} 
Here $Q_x\left(\cdot\vert x_t, a_t\right)$ represents the dynamics of the \mdp.  $V_{t+1}\left(\cdot\right)$ gives the value function at the future state and $\delta$ is the discounting parameter. Our algorithm is based on Expected Sarsa, which is a model free \rl algorithm that does not require the knowledge of model dynamics and produces a low variance estimate of the $Q$-value function.

Let us define an equilibrium generating function $\ttheta=(\ttheta^i_t)_{i\in\{l,f\},t\in[T]}$, where $\ttheta_t : \mathcal{P}(\cX) \to \left\{\cX \to \mathcal{P}(\cA^f) \right\} \times \mathcal{P}(\cA^l) $. In addition, we define value functions $\cm{V_t^f,V_t^l}$ and action value functions $(Q_t^l,Q_t^f)_{t\in \{ 1,2, \ldots T+1\}}$ , where 
\begin{align}
	V_t^f&: \mathcal{P}(\cX) \times \cX \to \mR\nn\\
	V_t^l&: \mathcal{P}(\cX) \to \mR\nn\\
	Q_t^f&: \mathcal{P}(\cX) \times \cX \times \cA \times \Gamma^f \to \mR\nn\\
	Q_t^l&: \mathcal{P}(\cX) \times \cA \times \Gamma^f \to \mR\nn
\end{align}

Here we describe the backward recursive algorithm that is used to compute the strategies using the value functions for each discrete value of the estimated belief state $\pih_t$.

\begin{enumerate}
	\item Initialize $\forall \pih_{T+1}\in \mathcal{P}(\cX), x_{T+1}\in \cX$,
	\begin{align}
		\label{eq:VT+1}
		V^f_{T+1}\cm{\pih_{T+1},x_{T+1}} &\defeq 0 \\
		V^l_{T+1}\cm{\pih_{T+1}} &\defeq 0 
	\end{align} 		
	\item For $t = T,T-1, \ldots 1, \ \forall \pih_t\in \mathcal{P}(\cX)$, let $\ttheta_t[\pih_t]$ be generated as follows. 
	
	$\forall \pih_t\in\Pi$, $x_t\in\cX$, $a_t\in\cA$ and $\tgamma^f_t\in K^{\gamma^f}$, compute $Q_t^l$ and $Q_t^f$ as
	\begin{align}
		\label{Eqn:Qdef1}
		Q_t^f\cm{\pih_t,x_t,a_t,\tgamma^f_t}&= \mE^\tau\Big[R_t^f\left(x_t,a_t\right) +\nn\\
		\delta V_{t+1}^f\Big(&\Fh^f\left(\pih_t, \tgamma^f_t, a_t\right), X_{t+1}\Big) \lvert x_t\Big]
	\end{align} 
	\begin{align}
		\label{Eqn:Qdef2}
		Q_t^l\cm{\pih_t,a_t,\tgamma^f_t}&= \mE^{\tau,\pih_t}\Big[R_t^l\left(X_t,a_t\right) +\nn\\
		\delta V_{t+1}^f&\left(\Fh^l\left(\pih_t, \tgamma^f_t, a_t\right)\right)\Big]
	\end{align} 
	where $\Fh\cm{\cdot}$ represents the particle filter function.

	Set $\tgamma_t = \ttheta_t[\pih_t]$, where $\tgamma_t =\cm{\tgamma_t^l,\tgamma_t^f}$ is the solution of the following fixed-point equation. 
	
	$\forall \gamma_t^l\in K^{\gamma^l}$, define $\Lambda(\gamma_t^l)$ as follows, $\forall x_t\in \cX$,
	\begin{align}
		\label{Eqn:fixed_point}
		&\Lambda_t^f(\gamma_t^l) =\Big\{\tgamma_t^f:\tgamma_t^f\in\nn\\
		&\arg\max_{\gamma^f_t\cm{\cdot\vert x_t}} \mE^{\gamma_t^f\cm{\cdot\vert x_t},\gamma_t^l}\sq{Q_t^f\cm{\pih_t,x_t,A_t,\tgamma^f_t}} \Big\}.
	\end{align}

	The solution to the strategy for the leader is compute using
	\begin{align}
	\label{Eqn:fixed_point2}
	\tgamma_t^l &\in \arg\max_{\gamma_t^l}\mE^{ \Lambda_t^f\left(\gamma_t^l\right){\gamma}^{l}_t} \sq{Q_t^l\cm{\pih_t,A_t,\tgamma^f_t}}
	\end{align}

	The solution to the above two steps generate $(\tgamma_t^l,\tgamma_t^f)$ as pair of equilibrium strategies.
	
	Now, we calculate the utility function values $\forall x_t\in\cX$,
	\begin{align}
	\label{Eqn:utility1}
		V^f_{t}\left(\pi_t,x_t\right) \defeq  &\;\mE^{\tilde{\gamma}^{f}_t\left(\cdot|x_t\right) \tilde{\gamma}^{l}_t,\, \pi_t}\left[{R}_t^f\left(x_t,A_t\right) + \right.\nn\\
								   			  &\left.\delta V_{t+1}^f \left(\Fh^f\left(\pi_t, \tilde{\gamma}^f_t, A_t\right), X_{t+1}\right)\big\lvert x_t \right]
	\end{align}
	and
	\begin{align}
	\label{Eqn:Utility2}
		V^l_{t}\left(\pi_t\right) \defeq  &\;\mE^{\tilde{\gamma}^{f}_t \tilde{\gamma}^{l}_t,\, \pi_t}\Big[ {R}_t^l\left(X_t,A_t\right) +\nn\\
							   &\delta V_{t+1}^l \left(\Fh^l\left(\pi_t, \tilde{\gamma}^f_t, A_t\right)\right) \Big].	
	\end{align}
\end{enumerate}

\subsubsection{Forward Recursion}

Based on $\ttheta$ defined in the backward recursion above, we now construct a set of strategies $\tsigma$ (through beliefs $\mu$) in a forward recursive way as follows. 
\begin{enumerate} 
	\item Initialize at time $t=1$, 
	\begin{align}
	\mu_1[\phi]\left(x_1\right) &:=  \tau\left(x_1\right). \label{eq:mu*def0}
	\end{align}
	
	\item For $t =1,2 \ldots T, \forall i =1,2, a_{1:t}\in \cH_{t+1}^c, x_{1:t} \in\cX^t$
	\begin{align}
	\label{Eqn:beta*def}
		\tsigma_{t}^{l}\left(a_{t}^l|a_{1:t-1}\right) &:= \ttheta_{t}^l\left[\mu_{t}\left[h_t^c\right]\right]\left(a^l_{t}\right) \\
		\tsigma_{t}^{f}\left(a_{t}^f|a_{1:t-1},x_{1:t}\right) &:= \ttheta_{t}^f\left[\mu_{t}\left[h_t^c\right]\right]\left(a^f_{t}|x_{t}\right)
	\end{align}
	\begin{align}
	\label{Eqn:mu*def}
		\mu_{t+1}\left[h_{t+1}^c\right] :=F\left(\mu_t\left[h_t^c\right], \ttheta_t^f\left[\mu_t\left[h_t^c\right]\right], a_t\right)
	\end{align}
\end{enumerate}
where $F$ is defined in \eqref{eq:F_update}.  

% %
% %We now state our main result.
% %
% %%%%%%%%%%%%

% A strategy and a belief profile $(\tsigma,\mu)$, as constructed through backward/forward recursion algorithm above is an \mpse of the game


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 	% where expectation in~\eqref{Eqn:fixed_point}) is with respect to $(A_t, X_{t+1})$ through the measure
	% $\gamma^f_t(a^f_t|x_t) {\gamma}^{l}_t(a^{l}_t)\tau(x_{t+1}|x_t,a_t)$ and $F$ is defined in Lemma~\ref{Lemma:belief_state}. 
	
% 	\item The solution to the strategy for the leader is compute using
% 	\begin{align}
% 	\label{Eqn:fixed_point2}
% 	\tgamma_t^l &\in \arg\max_{\gamma_t^l}\mE^{ \Lambda_t^f\left(\gamma_t^l\right){\gamma}^{l}_t,\,\pi_t} \left[R_t^l\left(X_t,A_t\right) +\right.\nn\\
% 				&\left.\delta V_{t+1}^l\left(F\left(\pi_t,  \Lambda_t^f\left(\gamma_t^l\right), A_t\right)\right)\right]
% 	\end{align}
% 	where the above expectation is defined with respect to random variables $(X_t,A_t)$ through the measure $\pi_t(x_t)\hat{\gamma}^f_t(a^f_t) {\gamma}^{l}_t(a^{l}_t)$, and $\hat{\gamma}_t\in \Lambda_t^f(\gamma_t^l)$.

% 	The solution to the above two steps generate $(\tgamma_t^l,\tgamma_t^f)$ as pair of equilibrium strategies.
	
% 	\item Now, we calculate the utility function values $\forall x_t\in\cX$,
% 	\begin{align}
% 	\label{Eqn:utility1}
% 		V^f_{t}\left(\pi_t,x_t\right) \defeq  &\;\mE^{\tilde{\gamma}^{f}_t\left(\cdot|x_t\right) \tilde{\gamma}^{l}_t,\, \pi_t}\left[{R}_t^f\left(x_t,A_t\right) + \right.\nn\\
% 								   			  &\left.\delta V_{t+1}^f \left(F\left(\pi_t, \tilde{\gamma}^f_t, A_t\right), X_{t+1}\right)\big\lvert x_t \right]
% 	\end{align}
% 	and
% 	\begin{align}
% 	\label{Eqn:Utility2}
% 		V^l_{t}\left(\pi_t\right) \defeq  &\;\mE^{\tilde{\gamma}^{f}_t \tilde{\gamma}^{l}_t,\, \pi_t}\left[ {R}_t^l\left(X_t,A_t\right) + \right.\nn\\
% 							   &\left.   \delta V_{t+1}^l \left(F\left(\pi_t, \tilde{\gamma}^f_t, A_t\right)\right) \right].	
% 	\end{align}
% \end{enumerate}

% \subsubsection{Forward Recursion}

% Based on $\ttttheta$ defined in the backward recursion above, we now construct a set of strategies $\tsigma$ (through beliefs $\mu$) in a forward recursive way as follows. 
% \begin{enumerate} 
% 	\item Initialize at time $t=1$, 
% 	\begin{align}
% 	\mu_1[\phi]\left(x_1\right) &:=  Q_x\left(x_1\right). \label{eq:mu*def0}
% 	\end{align}
	
% 	\item For $t =1,2 \ldots T, \forall i =1,2, a_{1:t}\in \cH_{t+1}^c, x_{1:t} \in\cX^t$
% 	\begin{align}
% 	\label{Eqn:beta*def}
% 		\tsigma_{t}^{l}\left(a_{t}^l|a_{1:t-1}\right) &:= \ttttheta_{t}^l\left[\mu_{t}\left[h_t^c\right]\right]\left(a^l_{t}\right) \\
% 		\tsigma_{t}^{f}\left(a_{t}^f|a_{1:t-1},x_{1:t}\right) &:= \ttttheta_{t}^f\left[\mu_{t}\left[h_t^c\right]\right]\left(a^f_{t}|x_{t}\right)
% 	\end{align}
% 	\begin{align}
% 	\label{Eqn:mu*def}
% 		\mu_{t+1}\left[h_{t+1}^c\right] :=F\left(\mu_t\left[h_t^c\right], \ttttheta_t^f\left[\mu_t\left[h_t^c\right]\right], a_t\right)
% 	\end{align}
% \end{enumerate}
% where $F$ is defined in \eqref{eq:F_update}.  
% %
% %We now state our main result.
% %
% %%%%%%%%%%%%

% A strategy and a belief profile $(\tsigma,\mu)$, as constructed through backward/forward recursion algorithm above is an \mpse of the game




==> STACKELBERG/4Algorithm.tex <==
In this section, we propose a model-free \rl algorithm based on Expected Sarsa~\cite{van2009theoretical} to compute the optimal \mpse strategy both for the leader and the follower. We follow the steps summarized in the sequential decomposition algorithm to derive these strategies. The algorithm iterates between the policy evaluation and policy improvement steps sequentially. At each instant $t$, and at each discretized belief state $\pih_t\in\Pi$, we compute $Q_t^i$ as in~\eqref{Eqn:Qdef1} and~\eqref{Eqn:Qdef2} using Expected Sarsa as a function of the equilibrium policy of the follower $\ttheta\sq{\pih_t}=\tgammatf$. This is essential in solving the fixed point equations for model free algorithms. Thereafter, we compute the optimal policies for the follower and the leader by solving the fixed point equation in~\eqref{Eqn:fixed_point} and the maximization in~\eqref{Eqn:fixed_point2} respectively. The value functions $V_t^f$ and $v_t^l$ are updated after the optimal policy $\ttheta_t$ is computed using the equations in~\eqref{Eqn:utility1} and~\eqref{Eqn:Utility2} to be used in the computation of $Q_t^i$ in the next iteration. 

\subsection{Policy Evaluation}

The $Q$-value functions $Q_{t}^f$ and $Q_{t}^l$ are computed from a sampled trajectory from the model bootstrapping it with the future value function $V_{t+1}^i$. It involves sampling from a model simulation of a generic player $i\in\left\{l,f\right\}$ which takes a current state $x_t\in\cX$ and actions $a_t\in\cA$, for every belief state $\pih_t$ and provides the next state $x_{t+1}$ and the corresponding reward $R_t^i(x_t, a_t)$. In the beginning of each iteration, the belief state estimate is updated to $\pih_{t+1}$ from the current estimated belief state $\pih_t$ at the equilibrium policy $\gamma_t^f$ by feeding the observation vector $a_t$ to the particle filter. It is computed separately for the follower and the leader as the model is not known to either of them. We use Expected Sarsa algorithm to update the $Q$-value for both the follower and the leader synchronously using the same simulated trajectory. Expected Sarsa follows the TD learning method where the update equation is given as
\begin{align}
	Q^f_t\cm{\pih_t,x_t,a_t,\tgamma_t^f} = \cm{1-\alpha}Q^f_t\cm{\pih_t,x_t,a_t,\tgamma_t^f}\nn\\ +\alpha \cm{R_t^f\cm{x_t,a_t}+\delta V_{t+1}^f\cm{\pih^f_{t+1},x_{t+1}}}
\end{align}
\begin{align}
	Q^l_t\cm{\pih_t,a_t,\tgamma_t^f} = \cm{1-\alpha}Q^l_t\cm{\pih_t,a_t,\tgamma_t^f}\nn\\ +\alpha \cm{\mE^{\pih_t}[R_t^l\cm{X_t,a_t}]+\delta V_{t+1}^l\cm{\pih^f_{t+1}}}
\end{align}
where $\left(x_t, a_t, x_{t+1}\right)$ are sampled from a simulated model and $\alpha$ is the learning parameter. We use linear interpolation to obtain $V_{t+1}^f\cm{\pih_{t+1},x_{t+1}}$, $V_{t+1}^l\cm{\pih_{t+1}}$ at a future state. The updated belief state is generated using the particle filter algorithm that was put forth in~\ref{sec:particle_filter}. It takes in the current belief state $\pih_{t}$, the follower's policy $\tgammatf$ and the observation $a_t$ and provides the empirical distribution $\pih_{t+1}$. 

\subsection{Policy Iteration}
\subsubsection{Follower Strategy}

The fixed point equation in \eqref{Eqn:fixed_point} is solved at the follower, for each discrete belief state $\pih_t\in\Pi$, to compute the follower's equilibrium strategy corresponding to each of the leader's strategy $\gamma_t^l\in\cK^{\gamma^l}$. Given the follower's $Q_t^f$-value function, the objective function for $x_t\in\cX$ with any strategy $\gamma_t^f$ can be expressed as

\begin{align}
	\label{Eqn:objective1}
	\tgammatf = \arg\max_{\gamma_t^f} \mE\sq{Q_{t}^f\cm{\pih_t, x_t, A_t,\gamma_t^f}}.
\end{align}

The expectation is taken over $A_t$ through the measure $\gamma_t^f\left(\cdot\vert x_t\right)\gamma_t^l\left(\cdot\right)$ representing the leader's strategy. It is solved by a continuous policy update in the direction of ascent of the gradient. This is achieved using any of the policy gradient approaches. In this paper, we use neural network based policy gradient method to compute the policies that maximize the gradient of the $Q_t^f$ value functions at any time $t$. Given that the the function $Q_t^f$ depends on the optimal policy, this process is repeated over iterations arriving at the required prescription function $\tgamma^f_t$. This is repeated at all the belief states $pih_t\in\Pi$ so that we get the final equilibrium function $\theta_t\left[\pih_t\right]$.

\subsubsection{Leader Strategy}

The leader, with the knowledge of the strategy set of the follower $\Lambda_t^f\left(\gamma_t^l\right)$, computed as a best response to its strategies, optimizes its own strategy by solving the maximization equation in \eqref{Eqn:fixed_point2} given as 
\begin{align}
	\label{Eqn:objective2}
	\tgammatl = \arg\max_{\gamma_t^l} \mE\sq{Q_{t}^f\cm{\pih_t, A_t, \gamma_t^f}}.
\end{align}
It is a known fact that this results in pure strategies. This implies that the solution could be easily computed as the greedy policy $\tgamma_t^l$ that has the highest $Q$ value for each belief $\pih_t$.


Finally, the equilibrium strategy is given by $\tilde{\gamma}_t = \theta_t[\pi_t]$, where $(\tgamma_t^l,\tgamma_t^f)$ and $\tgamma_t^f = BR_t^f\left(\gamma_t^l)\right)$. 

\begin{algorithm}[!tb]
	\label{alg:Optimal_Policy}
	\DontPrintSemicolon
	\SetAlgoLined
	\KwIn{$Q^f_{t}$, $Q^l_{t}\quad \forall \gamma^f_{t}\in{\cK}^{\gamma^f_{t}}$, $\pih_{t} \in \Pi$\newline
		$\theta_{t}\left[\pih_{t}\right]\quad \forall \pih_t\in\Pi$}
	\vspace{.1cm}
	\KwOut{$\ttheta$}
	\vspace{.1cm}
	Initialize: $V^f_{T+1}$, $V^l_{T+1}$\;
	\For{$t=T\ldots1$}
	{
		Evaluate: $Q_t^f = FollowerQ\cm{V_{t+1}^f}$\;
		Evaluate: $Q_t^l = LeaderQ\cm{V_{t+1}^l}$\;
		\For{$\pih_t\in\Pi$}
		{
			\For{$\gamma^l_t\in\Pi$}
			{
				Compute: $\Lambda\cm{\gamma_t^l} = PolicyF\cm{Q_t^f,\gamma_t^l}$\;
			}
			Compute: $\tgammatl = PolicyL\cm{Q_t^l}$\;
			$\tgammatf = \Lambda\cm{\tgammatl}$\;
			\For{$x_t\in\cX$}
			{
				$V_t^f\cm{\pih_t,x_t} = \mE^{\tgammatf,\tgammatl}\sq{Q_t^f\cm{\pih_t,x_t,A_t}}$\;				
			}
			$V_t^l = \mE^{\tgammatf,\tgammatl}\sq{Q_t^l\cm{\pih_t,A_t}}$\;
			$\ttheta\sq{\pih_t}=\tgammatf$, $\tgammatl$\;
		}
	}
	\KwResult{$\ttheta$}
	\caption{Optimal policy}
\end{algorithm}

\begin{algorithm}[!tb]
	\label{alg:Policy Evaluation}
	\DontPrintSemicolon
	\SetAlgoLined
	\KwIn{$V_{t+1}^f$, $V_{t+1}^l$, $\gamma_t^l$}
	\vspace{.1cm}
	\KwOut{$Q_t^f$, $Q_t^l$}
	\vspace{.1cm}
	\For{$\pi_t,\gamma_t^f\in\Pi\times{\cK}^{\gamma^f}$}
	{ 
		Initialize: $Q_t^f$, $Q_t^l$\;
		\For{$l=1\ldots L$}
		{
			\For{$a^f_t,a^l_t\in\cA^f\times\cA^l$}
			{
				$a_t=\cm{a_t^f,a_t^l}$\;
				\For{$x_t\in\cX$}
				{
					Sample: $x_{t+1}\sim \tau\cm{\cdot\vert x_t,a_t}$\;
					$\pih^f_{t+1} = PF\cm{\pi_t, \gamma_t^f, a_t}$\; 
					$T^f =  R_t^f\cm{x_t,a_t}+\delta V_{t+1}^f\cm{\pih^f_{t+1},x_{t+1}}$
					$R^l{x_t,a_t} = R_t^l\cm{x_t,a_t}$\;
					$Q^f_t\cm{\pi_t,x_t,a_t,\gamma_t^f} = \cm{1-\alpha}Q^f_t\cm{\pi_t,x_t,a_t,\gamma_t^f} + \alpha T^f$\;
				}
				$\pih^l_{t+1} = PF\cm{\pi_t, \gamma_t^f, a_t}$\;
				$T^l = \mE^{\pi_t}\sq{R^l\cm{X_t,a_t}} + V_{t+1}^l\cm{\pih_{t+1}}$\;
				$Q^l_t\cm{\pi_t, a_t,\gamma^f_t} = \cm{1-\alpha}Q^l_t\cm{\pi_t, a_t,\gamma^f_t} + \alpha T^l$\; 
			}
				
		} 
	
	}	
	\KwResult{$Q^f_t$, $Q^l_t$}
	\caption{Policy Evaluation ($Q$-value Estimation)}
\end{algorithm}

% \begin{algorithm}[!tb]
% 	\label{alg:Policy Evaluation}
% 	\DontPrintSemicolon
% 	\SetAlgoLined
% 	\KwIn{$Q^f_{t}$, $Q^l_{t}\quad \forall \gamma^f_{t}\in{\cK}^{\gamma^f_{t}}$, $\pi_{t} \in \Pi$\newline
% 		$\theta_{t}\left[\pi_{t}\right]\quad \forall \pi_t\in\Pi$}
% 	\vspace{.1cm}
% 	\KwOut{$Q^f_{t-1}$, $Q^l_{t-1}\quad \forall \gamma_{t-1}\in{\cK}^{\gamma_{t-1}}$, $\pi_{t-1} \in \Pi$}
% 	\vspace{.1cm}
% 	\For{$\pi_{t-1},\gamma^f_{t-1}\in\Pi\times{\cK}^{\gamma^f_{t-1}}$}{ 
% 		$Q_{t-1}^f\left(\pi_{t-1},x_{t-1}, a_{t-1},\gamma^f_{t-1}\right) = Q^f_{t}\left(\pi_{t-1},x_{t-1},a_{t-1},\gamma_{t-1}^f\right)$\;
% 		$Q_{t-1}^l\left(\pi_{t-1},a^l_{t-1},\gamma^f_{t-1}\right) = Q^l_{t}\left(\pi_{t-1},a^l_{t-1},\gamma_{t-1}^f\right)$\;
% 			\For{$a^l_{t-1}\in\cA^l$}{
% 				\For{$\left(x_{t-1},a^f_{t-1}\right)\in\cX\times\cA^f$}{
% 					$a_{t-1}=\left(a_{t-1}^f,a_{t-1}^l\right)$\;
% 					Sample: $x_{t}\sim Q_x\left(.\vert x_{t-1},a_{t-1},\gamma_{t-1}^f\right)$\;
% 					$\pi_{t}^f=$ Belief Update$\left(\pi_{t-1}, \gamma_{t-1}^f, a_{t-1} \right)$\; 
% 					$\pi_{t}^l=$ Belief Update$\left(\pi_{t-1}, \gamma_{t-1}^f, a_{t-1} \right)$\; 
% 					$\tgammatf,\tgammatl = \theta_{t}\left[\pi^f_{t}\right]$\;
% 					$V_{t}^f = \mE^{\tgamma^f_t,\tgamma^l_t}\left[Q^f_{t}\left(\pi^f_{t},x_t,A_t,\tgamma_{t}^f\right)|x_t\right]$\;
% 					$\tgammatf,\tgammatl = \theta_{t}\left[\pi^l_{t}\right]$\;
% 					$V_{t}^l = \mE^{\tgamma^l_t}\left[Q^l_{t}\left(\pi^l_{t},A^l_t, \tgamma_{t}^f\right)\right]$\; 		
% 					$Q^f_{n} = R_{t-1}^f\left(x_{t-1},a_{t-1}\right)+\delta V_t^f$\;
% 					$Q^l_{n}\left(x_{t-1},a^f_{t-1}\right) = R_{t-1}^l\left(x_{t-1},a_{t-1}\right)+\delta V_t^l$\;
% 					$Q^f_{t-1}\left(\pi_{t-1},x_{t-1}, a_{t-1},\gamma^f_{t-1}\right) = \left(1-\alpha\right)Q^f_{t-1}\left(\pi_{t-1},x_{t-1}, a_{t-1},\gamma^f_{t-1}\right) + \alpha Q^f_{n}$\; 
% 				}
% 				$Q^l_{t-1}\left(\pi_{t-1}, a^l_{t-1},\gamma^f_{t-1}\right) = \left(1-\alpha\right)Q^l_{t-1}\left(\pi_{t-1}, a^l_{t-1},\gamma^f_{t-1}\right) + \alpha \mE^{\gamma_{t-1}^f,\pi_{t-1}}\left[Q^l_{n}\left(X_{t-1},A^f_{t-1}\right)\right]$\; 
				
% 			} 
		
% 		}	
% 	\KwResult{$Q^f_{t-1}$, $Q^l_{t-1}$}
% 	\caption{Policy Evaluation ($Q$-value Estimation)}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \label{sec:Algo}
% In this section, we propose a model-free \rl algorithm, based on Expected Sarsa~(\cite{van2009theoretical}) and the backward recursion presented in the previous section, to compute the optimal \mpse strategy both for the leader and the follower. 

% In a general \rl setting, with finite state space $\cX$ and finite action space $\cA$, we can express the $Q$-value for the state action pair $\left(x_t, a_t\right)$ for all $x_t\in\cX$, $a_t\in\cA$ in terms of the reward $R_t\left(x_t, a_t\right)$ as
% \begin{align}
% \label{Eqn:Bellman_optimality}
% 	Q_t\left(x_t, a_t\right)=R_t\left(x_t, a_t\right)+\delta\mE^{Q_x}\left[V_{t+1}\left(X_{t+1}\right)\right]. 
% \end{align} 
% Here $Q_x\left(\cdot\vert x_t, a_t\right)$ represents the dynamics of the \mdp. $V_{t+1}\left(\cdot\right)$ gives the value function at the future state and $\delta$ is the discounting parameter. Our algorithm is based on Expected Sarsa, which is a model-free \rl algorithm that does not require the knowledge of model dynamics and produces a low variance estimate of the $Q$-value function.

% In the Stackelberg game that we consider, the \rl setting for the follower and the leader differ as detailed in Section~\ref{sec:Model}. The $Q$-value function for the follower depends on the private type $x_t$ and belief state $\pi_t$ along with the common action $a_t$. Also, the action $a_t$ at any state $\left(x_t, \pi_t\right)$ results in a future state $\left(x_{t+1}, \pi_{t+1}\right)$ which is a function of the follower's policy as given in Lemma~\ref{Lemma:belief_state}. Therefore, we define the $Q$-value function for the follower as $Q_t^f:\cX\times\Pi\times\cA\times{\cK}^{\gamma^f}\rightarrow\mR$, where ${\cK}^{\gamma^f}$ represents the space spanned by $\gamma_t^f$. Similarly, in case of a leader, which has no private information, the $Q$-value function is defined as $Q_t^l:\Pi\times\cA^l\times{\cK}^{\gamma^f}\rightarrow\mR$. We now proceed to reformulate the equations in~\eqref{Eqn:fixed_point} and~\eqref{Eqn:fixed_point2} in the backward recursion algorithm in terms of the newly defined $Q$-value functions and get,
% \begin{align}
% \label{Eqn:fixed_point_changed}
% &BR_t^f(\gamma_t^l) =\nn\\
% 	&\left\{ \tgamma_t^f: \tgamma_t^f\in \arg\max_{\gamma^f_t}\mE\left[Q_{t}^f\left(\pi_{t}, x_t, A_{t},\tgamma^f_t\right)\right]  \right\}
% \end{align}
% and 
% \begin{align}
% 	\label{Eqn:fixed_point_changed2}
% 	\tgamma_t^l \in \arg\max_{\gamma_t^l}\mE\left[Q_{t}^l\left(\pi_{t}, A^l_{t},\tgamma_t^f\right)\right]
% \end{align}
% for the follower and the leader respectively. Here
% \begin{align}
% 	\label{Eqn:Q_follower}
% 	Q_t^f = \mE\left[R_t^f\left(x_t, a_t\right) +\delta V_{t+1}^f\left(\pi_{t+1}, X_{t+1}\right)\right]
% \end{align}
% and
% \begin{align}
% 	\label{Eqn:Q_leader}
% 	Q_t^l= \mE\left[R_t^f\left(X_t,A_t^f, a_t^l\right) +\delta V_{t+1}^l\left(\pi_{t+1}, X_{t+1}\right)\right].
% \end{align}
% The expectation in~\eqref{Eqn:fixed_point_changed} is with respect to random variable $A_t$ through the measure $\gamma^f_t(a^f_t|x_t) {\gamma}^{l}_t(a^{l}_t)$ while the expectation in~\eqref{Eqn:fixed_point_changed2} is with respect to random variable $A_t^l$ through the measure ${\gamma}^{l}_t(a^{l}_t)$. The expectation in \eqref{Eqn:Q_follower} is on next state $X_{t+1}$ through the \mdp dynamics $Q_x(x_{t+1}|x_t,a_t)$. The updated belief state $\pi_{t+1}$ is as defined in Lemma~\ref{Lemma:belief_state}. 
 
% We follow the steps summarized in the sequential decomposition algorithm to derive the equilibrium strategies. At time $T$, we initialize the $Q$-values and the equilibrium strategies $\theta_T[\pi_T]$ as $0$. Then, we use the formulations described in~\eqref{Eqn:fixed_point_changed}-\eqref{Eqn:Q_leader} to update the equilibrium strategy $\tilde{\gamma}_T = \theta_T[\pi_T]$, where $(\tgamma_T^l,\tgamma_T^f)$ and $\tgamma_T^f = BR_T^f\left(\tgamma_T^l)\right)$ corresponding to all $\pi_{T}\in\Pi$. Subsequently, we use the updated strategies and a modified low variance Expected Sarsa algorithm to estimate the $Q$-value, $Q^i_{T-1}$ for $i\in\{l,f\}$ for the previous time step $T-1$ for all follower strategies spanning $\cK^{\gamma^f}$. These $Q$-values are then used to obtain the equilibrium strategies for the follower and the leader at time $T-1$ as before. This sequence is repeated for all time instants $T,T-1,\ldots 1$. Basically, our algorithm iterates between policy iteration and policy evaluation, which are discussed in details below.

% \subsection{Policy Iteration}
% \subsubsection{Follower Strategy}
% At any time $t$, the fixed point equation in \eqref{Eqn:fixed_point_changed} is solved at the follower, for each discrete belief state $\pi_t\in\Pi$, to compute the follower's equilibrium strategy corresponding to each of the leader's strategy $\gamma_t^l\in\cK^{\gamma^l}$. Given the follower's $Q$-value function $Q_t^f$, the value function for any type $x_t\in\cX$ with any strategy $\gamma_t^f$ can be calculated as
% \begin{align}
% 	\label{Eqn:objective_value}
% 	V_t^f\left(x_t,\pi_t\right) =  \mE\left[Q_{t}^f\left(x_t,A_t,\pi_t, \gamma_t^f\right)\right].
% \end{align}
% The expectation is taken over $A_t$ through the measure $\gamma_t^f\left(\cdot\vert x_t\right)\gamma_t^l\left(\cdot\right)$ representing the leader's strategy. At each iteration, linear interpolation is used as a form of function approximation to estimate the $Q$-value at any given value of $\pi_t$ and $\gamma_t^f$. The strategy $\gamma_t^f$ is then updated so as to maximize~\eqref{Eqn:objective} given as
% \begin{align}
% 	\label{Eqn:objective}
% 	\tgammatf = \arg\max_{\gamma_t^f} V_t^f\left(x_t,\pi_t\right)
% \end{align}
% which is the same fixed point equation as in~\eqref{Eqn:fixed_point}. It is solved by a continuous policy update in the direction of ascent of the gradient represented as some function $f$ which could be chosen by any standard method with any appropriate $\beta$ value. The function $f$ should satisfy the constraint of probability measures to ensure convergence. The steps in the computation can be summarized as below.
% \begin{align}
% 	q^f_n\left(x_t, a_t^f\right)  &= \mE^{\gamma_t^l}\left[Q_{t}^f\left(x_t,a_t^f, A_t^l, \pi_t, \gamma_n^f\right)\right]\label{Eqn:update1}\\
% 	v^f_n &= \mE^{\gamma_t^f\left(\cdot\vert x_t\right)}\left[q_n\left(x_t, A_t^f\right)\right]\label{Eqn:update2}\\
% 	\Delta\gamma &= f\left(v^f_n, \bar{q}^f_n\right)\label{Eqn:update3}\\
% 	\gamma^f_{n+1} &= \gamma_n^f + \beta\Delta\gamma\label{Eqn:update4}
% \end{align}

% Iterating over the steps~\eqref{Eqn:update1}-\eqref{Eqn:update4}, we update the strategy $\gamma_t^f$ until it stabilizes which gives the final equilibrium strategy $\tgammatf$ as the best response to the leader's strategy $\gamma_t^l$. This process is repeated for all possible equilibrium strategies of the leader $\gamma_t^l\in\cK^{\gamma_t^l}$ for all $\pi_t\in\Pi$ to arrive at the set $BR_t^f\left(\gamma_t^l\right)$. $\bar{q}^f_n$ represents a vector containing the $Q$-values calculated at all possible actions $a_t^f\in\cA$ using~\eqref{Eqn:update1}.

% \subsubsection{Leader Strategy}
% The leader, with the knowledge of the strategy set of the follower $BR_t^f\left(\gamma_t^l\right)$, computed as a best response to its strategies, optimizes its own strategy by solving the maximization equation in \eqref{Eqn:fixed_point_changed2}. This is done by comparing the strategies such that the resulting value at the future state becomes indifferent to the action taken at the current state or in other words, the final value function of the state yields equal values for all the possible actions is taken based on the strategy. The $Q$-value for the leader is estimated using linear interpolation similar to the follower, for a particular belief state $\pi_t$ as
% \begin{align}
% \label{Eqn:objective_value1}
% q^l\left(a_t^l\right) &=  Q_{t}^l\left(a_t^l,\pi_t, BR_t^f\left(\gamma_t^l\right)\right)\\
% v^l &= \mE^{\gamma_t^l}\left[q^l\left(A_t^l\right)\right]
% \end{align}
% The equilibrium policy $\gamma_t^l$ that makes $v^l$ exceed over $q^l\left(a_t^l\right)$ for all $a_t^l\in\cA^l$ forms the solution to the maximization problem. Finally, the equilibrium strategy is given by $\tilde{\gamma}_t = \theta_t[\pi_t]$, where $(\tgamma_t^l,\tgamma_t^f)$ and $\tgamma_t^f = BR_t^f\left(\gamma_t^l)\right)$. 

% \subsection{Policy Evaluation}

% The $Q$-value functions $Q_{t}^f$ and $Q_{t}^l$, which were used to compute the equilibrium policies, have to be estimated by sampling from a model simulation of a generic agent $i\in\left\{l,f\right\}$ that takes a current state $x_t\in\cX$ and actions $a_t^i\in\cA^i$, for every belief state $\pi_t$ and provides the next state $x_{t+1}$ and the corresponding reward $R_t^i(x_t, a_t)$. We have already discussed the policy iteration method that computes the equilibrium policies $\theta_{t}\left[\pi_t\right]\forall\pi_t\in\Pi$ for both the follower and the leader. Using these policies and the already estimated values of $Q_{t}^i$ at time $t$, the new values $Q_{t-1}^i$ at time $t-1$ are estimated $\forall \gamma_{t-1}^f\in\cK^{\gamma^f}$.

% In the beginning of each iteration, the belief state was updated to $\pi_{t+1}$ from the current belief state $\pi_t$ at the equilibrium policy $\gamma_t^f$. It is computed separately for the follower and the leader as the model is not known to either of them. They rely on Monte Carlo sampling to obtain the Bayesian update using an algorithm referred as particle filter, which is discussed later. We use Expected Sarsa algorithm to update the $Q$-value for both the follower and the leader synchronously using the same simulated trajectory. Expected Sarsa follows the TD learning method where the update equation is given as
% \begin{align}
% Q\left(x_t,a_t\right) = \left(1-\alpha\right)Q\left(x_t,a_t\right) +\nn\\ \alpha\left(R\left(x_t, a_t\right)+\delta V\left(x_{t+1}\right)\right)
% \end{align}
% where $\left(x_t, a_t, x_{t+1}\right)$ are sampled from a simulated model. The learning parameter $\alpha$ is carefully chosen to be $\frac{1}{\#\left(x_l^i,a_l^i\right)^{0.5-1}}$ to guarantee convergence in polynomial time~(\cite{even2003learning}). The value $\#\left(x_l^i,a_l^i\right)$ denotes the number of times the particular $\left(x_t,a_t\right)$ is encountered.

% The overall algorithm shown in Algorithm~\ref{alg:Policy Evaluation}, iterates over the policy iteration and policy evaluation sequentially to arrive at the equilibrium strategy. Multiple batch updates could be carried out to estimate $Q_t^f$ and $Q_t^l$ in a single iteration of policy evaluation. However, in the algorithm shown, we just consider a single batch update for convenient representation. The policy evaluation serves to refine the estimate for the equilibrium strategy so that at the end of the policy iteration, the overall expected returns is maximized.
% \subsubsection{Updating Belief State}

% The evolution of the belief state $\pi_t$ is given by Lemma~\ref{Lemma:belief_state} and~\eqref{eq:F_update}. The equation, however, uses the transition probability of the \mdp to get the updated belief value. Here we demonstrate a method to estimate the future update $\pi_{t+1}$ from the current belief $\pi_t$~(\cite{silver2010monte}). The algorithm is called a particle filter. The belief state is approximated using $K$ simulated particles as $B_{t}^i\in\cX,1\leq i\leq K$ such that the belief state for $x_{t}$ can be computed as

% \begin{align}
% 	\label{Eqn:pi_update}
% 	\pi_{t+1}\left(x_{t}\right)=\frac{1}{K}\sum_i\delta_{x_{t}B_{t}^i}
% 	\end{align}
% 	where $\delta_{xx^\prime}$ represents the Kronecker delta function. Algorithm~\ref{alg:Belief Update} illustrates the method to find the updated belief state set. The updated belief for any $x_{t+1}$ is computed as in~\eqref{Eqn:pi_update}. 
% \begin{align}
% 	\label{Eqn:pi_update}
% 	\pi_{t+1}\left(x_{t}\right)=\frac{1}{K}\sum_i\delta_{x_{t}B_{t}^i}
% 	\end{align}
% 	where $\delta_{xx^\prime}$ represents the Kronecker delta function. Algorithm~\ref{alg:Belief Update} illustrates the method to find the updated belief state set. The updated belief for any $x_{t+1}$ is computed as in~\eqref{Eqn:pi_update}. 

% \begin{algorithm}[!tb]
% 	\label{alg:Optimal_Policy}
% 	\DontPrintSemicolon
% 	\SetAlgoLined
% 	\KwIn{$Q^f_{t}$, $Q^l_{t}\quad \forall \gamma^f_{t}\in{\cK}^{\gamma^f_{t}}$, $\pi_{t} \in \Pi$\newline
% 		$\theta_{t}\left[\pi_{t}\right]\quad \forall \pi_t\in\Pi$}
% 	\vspace{.1cm}
% 	\KwOut{$\ttheta$}
% 	\vspace{.1cm}
% 	Initialize: $V^f_{T+1}$, $V^l_{T+1}$\;
% 	\For{$t=T\ldots1$}
% 	{
% 		Evaluate: $Q_t^f = FollowerQ\cm{V_{t+1}^f}$\;
% 		Evaluate: $Q_t^l = LeaderQ\cm{V_{t+1}^l}$\;
% 		\For{$\pi_t\in\Pi$}
% 		{
% 			\For{$\gamma^l_t\in\Pi$}
% 			{
% 				Compute: $\Lambda\cm{\gamma_t^l} = PolicyF\cm{Q_t^f,\gamma_t^l}$\;
% 			}
% 			Compute: $\tgammatl = PolicyL\cm{Q_t^l}$\;
% 			$\tgammatf = \Lambda\cm{\tgammatl}$\;
% 			\For{$x_t\in\cX$}
% 			{
% 				$V_t^f\cm{\pi_t,x_t} = \mE^{\tgammatf,\tgammatl}\sq{Q_t^f\cm{\pi_t,x_t,A_t}}$\;				
% 			}
% 			$V_t^l = \mE^{\tgammatf,\tgammatl}\sq{Q_t^l\cm{\pi_t,A_t}}$\;
% 			$\ttheta\sq{\pi_t}=\tgammatf$, $\tgammatl$\;
% 		}
% 	}
% 	\KwResult{$\ttheta$}
% 	\caption{Optimal policy)}
% \end{algorithm}

% \begin{algorithm}[!tb]
% 	\label{alg:Policy Evaluation}
% 	\DontPrintSemicolon
% 	\SetAlgoLined
% 	\KwIn{$V_{t+1}^f$, $V_{t+1}^l$, $\gamma_t^l$}
% 	\vspace{.1cm}
% 	\KwOut{$Q_t^f$, $Q_t^l$}
% 	\vspace{.1cm}
% 	\For{$\pi_t,\gamma_t^f\in\Pi\times{\cK}^{\gamma^f}$}
% 	{ 
% 		Initialize: $Q_t^f$, $Q_t^l$\;
% 		\For{$l=1\ldots L$}
% 		{
% 			\For{$a^f_t,a^l_t\in\cA^f\times\cA^l$}
% 			{
% 				$a_t=\cm{a_t^f,a_t^l}$\;
% 				\For{$x_t\in\cX$}
% 				{
% 					Sample: $x_{t+1}\sim \tau\cm{\cdot\vert x_t,a_t}$\;
% 					$\pih^f_{t+1} = PF\cm{\pi_t, \gamma_t^f, a_t}$\; 
% 					$T^f =  R_t^f\cm{x_t,a_t}+\delta V_{t+1}^f\cm{\pih^f_{t+1},x_{t+1}}$
% 					$R^l{x_t,a_t} = R_t^l\cm{x_t,a_t}$\;
% 					$Q^f_t\cm{\pi_t,x_t,a_t,\gamma_t^f} = \cm{1-\alpha}Q^f_t\cm{\pi_t,x_t,a_t,\gamma_t^f} + \alpha T^f$\;
% 				}
% 				$\pih^l_{t+1} = PF\cm{\pi_t, \gamma_t^f, a_t}$\;
% 				$T^l = \mE^{\pi_t}\sq{R^l\cm{X_t,a_t}} + V_{t+1}^l\cm{\pih_{t+1}}$\;
% 				$Q^l_t\cm{\pi_t, a_t,\gamma^f_t} = \cm{1-\alpha}Q^l_t\cm{\pi_t, a_t,\gamma^f_t} + \alpha T^l$\; 
% 			}
				
% 		} 
	
% 	}	
% 	\KwResult{$Q^f_t$, $Q^l_t$}
% 	\caption{Policy Evaluation ($Q$-value Estimation)}
% \end{algorithm}
	

% \begin{algorithm}[!htb]
% 	\label{alg:Belief Update}
% 	\DontPrintSemicolon
% 	\SetAlgoLined
% 	\KwIn{$\pi_{t}$,$\tgammatf$,$a_t$}
% 	\vspace{.1cm}
% 	\KwOut{$\pi_{t+1}$}
% 	\vspace{.1cm}
% 	$B_{t}^i\in\cX,1\leq i\leq K$\;
% 	\For{$K$ particles}
% 	{
% 		Sample: $x_t\sim B_t$\;
% 		Sample: $a_t^f\sim\tgammatf\left(\cdot\vert x_t\right)$\;
% 		Sample: $x_{t+1}\sim Q_x\left(\cdot\vert x_t, a_t^f\right)$\;
% 		\If{$a_t^f==a_t$}
% 		{
% 			Add: $x_{t+1}$ to $B_{t+1}$\;
% 		}
% 	}	
% $\pi_{t+1} = \frac{1}{K}\sum_i\delta_{xB_{t+1}^i}\quad\forall x\in\cX$\;
% 	\KwResult{$\pi_{t+1}$}
% 	\caption{Particle Filter (Belief Update)}
% \end{algorithm}



% % \begin{algorithm}[!tb]
% % 	\label{alg:Policy Evaluation}
% % 	\DontPrintSemicolon
% % 	\SetAlgoLined
% % 	\KwIn{$Q^f_{t}$, $Q^l_{t}\quad \forall \gamma^f_{t}\in{\cK}^{\gamma^f_{t}}$, $\pi_{t} \in \Pi$\newline
% % 		$\theta_{t}\left[\pi_{t}\right]\quad \forall \pi_t\in\Pi$}
% % 	\vspace{.1cm}
% % 	\KwOut{$Q^f_{t-1}$, $Q^l_{t-1}\quad \forall \gamma_{t-1}\in{\cK}^{\gamma_{t-1}}$, $\pi_{t-1} \in \Pi$}
% % 	\vspace{.1cm}
% % 	\For{$\pi_{t-1},\gamma^f_{t-1}\in\Pi\times{\cK}^{\gamma^f_{t-1}}$}{ 
% % 		$Q_{t-1}^f\left(\pi_{t-1},x_{t-1}, a_{t-1},\gamma^f_{t-1}\right) = Q^f_{t}\left(\pi_{t-1},x_{t-1},a_{t-1},\gamma_{t-1}^f\right)$\;
% % 		$Q_{t-1}^l\left(\pi_{t-1},a^l_{t-1},\gamma^f_{t-1}\right) = Q^l_{t}\left(\pi_{t-1},a^l_{t-1},\gamma_{t-1}^f\right)$\;
% % 			\For{$a^l_{t-1}\in\cA^l$}{
% % 				\For{$\left(x_{t-1},a^f_{t-1}\right)\in\cX\times\cA^f$}{
% % 					$a_{t-1}=\left(a_{t-1}^f,a_{t-1}^l\right)$\;
% % 					Sample: $x_{t}\sim Q_x\left(.\vert x_{t-1},a_{t-1},\gamma_{t-1}^f\right)$\;
% % 					$\pi_{t}^f=$ Belief Update$\left(\pi_{t-1}, \gamma_{t-1}^f, a_{t-1} \right)$\; 
% % 					$\pi_{t}^l=$ Belief Update$\left(\pi_{t-1}, \gamma_{t-1}^f, a_{t-1} \right)$\; 
% % 					$\tgammatf,\tgammatl = \theta_{t}\left[\pi^f_{t}\right]$\;
% % 					$V_{t}^f = \mE^{\tgamma^f_t,\tgamma^l_t}\left[Q^f_{t}\left(\pi^f_{t},x_t,A_t,\tgamma_{t}^f\right)|x_t\right]$\;
% % 					$\tgammatf,\tgammatl = \theta_{t}\left[\pi^l_{t}\right]$\;
% % 					$V_{t}^l = \mE^{\tgamma^l_t}\left[Q^l_{t}\left(\pi^l_{t},A^l_t, \tgamma_{t}^f\right)\right]$\; 		
% % 					$Q^f_{n} = R_{t-1}^f\left(x_{t-1},a_{t-1}\right)+\delta V_t^f$\;
% % 					$Q^l_{n}\left(x_{t-1},a^f_{t-1}\right) = R_{t-1}^l\left(x_{t-1},a_{t-1}\right)+\delta V_t^l$\;
% % 					$Q^f_{t-1}\left(\pi_{t-1},x_{t-1}, a_{t-1},\gamma^f_{t-1}\right) = \left(1-\alpha\right)Q^f_{t-1}\left(\pi_{t-1},x_{t-1}, a_{t-1},\gamma^f_{t-1}\right) + \alpha Q^f_{n}$\; 
% % 				}
% % 				$Q^l_{t-1}\left(\pi_{t-1}, a^l_{t-1},\gamma^f_{t-1}\right) = \left(1-\alpha\right)Q^l_{t-1}\left(\pi_{t-1}, a^l_{t-1},\gamma^f_{t-1}\right) + \alpha \mE^{\gamma_{t-1}^f,\pi_{t-1}}\left[Q^l_{n}\left(X_{t-1},A^f_{t-1}\right)\right]$\; 
				
% % 			} 
		
% % 		}	
% % 	\KwResult{$Q^f_{t-1}$, $Q^l_{t-1}$}
% % 	\caption{Policy Evaluation ($Q$-value Estimation)}
% % \end{algorithm}


==> STACKELBERG/5Convergence.tex <==

In this section, we prove the convergence of the proposed \rl algorithm to the equilibrium strategy of the statistical Stackelberg equilibrium. We put forth the following theorem.
\begin{theorem}
	The policies $\tsigma=\cm{\tsigma^f,\tsigma^l}$ thus generated from the \rl algorithm using the particle filter does form a $\epsilon$-\mpse of the Stackelberg game i.e.
	For the follower, we show,
	\begin{align}
		\label{Eqn:follower_1}
		J^{f,\tsigma^f,\tsigma^l}_t + \epsilon_t \geq J^{f,\sigma^f,\tsigma^l}_t
	\end{align}
	and for the leader we show,
	\begin{align}
		\label{Eqn:leader_1}
		J^{l,\tsigma^f,\tsigma^l}_t + \epsilon_t \geq J^{f,\Lambda\cm{\sigma^l},\sigma^l}_t.
	\end{align}

	\begin{proof}
		The proof to~\eqref{Eqn:follower_1} has been shown in Theorem~\ref{Thm:main_theorem} while the proof to~\eqref{Eqn:leader_1} has been shown in Theorem~\ref{Thm:main_theorem1}.
	\end{proof}

\end{theorem}
 

\begin{lemma} \label{Lemma:V_pf}
	The worst case error in the value function if we use a particle filter to update the belief state can be expressed as
	\begin{align}
		\label{Eqn:lemma2_to_prove}
		\Vert V^i_t\left(\pih_t,x_t^i\right) - {V^\star}^i_t\left(\pi_t,x_t^i\right)\Vert \leq \epsilon_1
	\end{align}
	where $\pi_t = \mu_t[1:a_{1-1}]$ and $\pih_t = \muh_t[1:a_{1-1}]$ are the belief trajectories with and without the particle filters.

	\begin{proof}
		This could be proved by using the Chernoff-Hoeffding bounds for deviation between sum of independent random variables from their true expectation. We leave the complete proof for the online version~\cite{schmidt1995chernoff}.

		It is also worth noting that the the value $epsilon$ is a function of the length of the time horizon and the discount factor. Moreover, it goes down with the increase in the number of particles used by the particle filter to estimate the belief. In our paper, we invariably choose a large $K$.
	\end{proof}
\end{lemma}

\subsection{Convergence of the Follower}
We put forth two lemmas that is used to prove the theorems. The lemmas have not been proven in this section due to lack of space but could be referred from the online version. 
\begin{lemma} 
	\label{Lemma:V_optimal_returns1}
	$\forall t\in\sq{T}$, $\forall \muh_t$ and $x_t\in\cX$,
	\begin{align}
		V_t^f\cm{\pih_t, x_t}= J^{f,\tsigma^f,\tsigma^f,\pih}_t
	\end{align}
	where $\tsigma_t=\cm{\tsigma^f_t,\tsigma_t^l}$ is the optimal policy at time $t$, $\pih_t = \muh_t[1:a_{1-1}]$ and $J_{t}$ is the accumulated optimal returns from $t$ till $T$.  
\end{lemma}

\begin{lemma} \label{Lemma:V_is_better1}
	$\forall t\in\cT$,$\forall \cm{a_{1:t-1},x_{1:t}}\in\cH_t^f$, $\sigma_t^f$,
	\begin{align}
		\label{Eqn:lemma2_to_prove1}
		{V_t^\star}^f\left(\pi_t,x_t\right) \geq \mE^{\sigma_t^f,\tsigma_{t}^l,\pi_t}\left[{Q^\star}^f_{t}\left(\pi_t, X_t, A_t,\tgamma^f_{t}\right)\right]
	\end{align}
	where $\pi_t = \mu_t[1:a_{1-1}]$ and $V^\star$ and $Q^\star$ represent the value functions in the case where model is known.
\end{lemma}

\begin{theorem}\label{Thm:main_theorem}
	A strategy $(\tilde{\sigma})$ constructed from the above algorithm is an $\epsilon$-\mpse of the game. i.e
	\begin{align}
		\label{Eqn:follower_main}
		J^{f,\tsigma^f,\tsigma^l,\pih_t}_t + \epsilon_2 \geq J^{f,\sigma^f,\tsigma^l,\pi_t}_t
	\end{align}

	We prove it through the technique of mathematical induction and will use the results that were proved before in Lemma~\ref{Lemma:V_optimal_returns2} and Lemma~\ref{Lemma:V_is_better2}.

	\begin{proof}
	For the base case, we consider $t = T$. The expected sum of returns, when the player $i$ follows the equilibrium policy $\tsigma$ is given as
	\begin{align}
			J_T^{f,\tsigma^f,\tsigma^l,\pi} = {V^\star}_T^f\left(\pi_T,x_T\right),\\
			J_T^{f,\tsigma^f,\tsigma^l,\pih} = V_T^f\left(\pih_T,x_T\right),
		\end{align}
		which is true from Lemma~\ref{Lemma:V_optimal_returns1}.
	From Lemma~\ref{Lemma:V_pf}, 
	\begin{align}
		\label{Eqn:follower_thm1}
		{V^\star}_T^f\left(\pi_T,x_T\right) \leq  V_T^f\left(\pih_T,x_T\right) + \epsilon
	\end{align}
	for some chosen small $\epsilon_T$. 
	From Lemma~\ref{Lemma:V_is_better2} and~\eqref{Eqn:follower_thm1} we get 
	\begin{align}
		J^{f,\tsigma^f,\tsigma^l,\pih_T}_T + \epsilon_T \geq J^{f,\sigma^f,\tsigma^l,\pi_T}_T
	\end{align}
		Assuming that the condition in~\eqref{Eqn:follower_main} holds at $t = t+1$, we get,
		\begin{align}
			\label{Eqn:assumption1}
			J^{f,\tsigma^f,\tsigma^l,\pih_{t+1}}_{t+1} + \epsilon_{t+1} \geq J^{f,\sigma^f,\tsigma^l,\pi_t}_{t+1}
		\end{align}
		We need to prove that the expression in~\eqref{Eqn:follower_main} holds for $t=t$ as well. 

		\begin{align}
			&J^{f,\tsigma^f,\tsigma^l,\pih_{t}}_{t}\label{Eqn:thm_le1}\\
			&=V^f_t\cm{\pih_t,x_t}\label{Eqn:thm_follower2}\\
			&\geq{V^\star}^f_t\cm{\pi_t,x_t} - \epsilon_{t+1}\label{Eqn:thm_follower3}\\
			&\geq\mE^{\sigma_t^f,\tsigma_{t}^l,\pi_t}\left[{Q_t^\star}^f\left(\pi_t, x_t, A_t, \tgamma^f_{t}\right)\right]- \epsilon_{t+1}\label{Eqn:thm_follower4}\\
			&=\mE^{\sigma_t^f,\tsigma_{t}^l,\pi_t}\left[R^f(x_t,a_t) + \delta {V^\star}^f_{t+1}\cm{\pi_{t+1},x_{t+1}}\right]- \epsilon_{t+1}\label{Eqn:thm_follower5}\\
			&\geq\mE^{\sigma_t^f,\tsigma_{t}^l,\pi_t}\left[R^f(x_t,a_t) + \delta {V}^f_{t+1}\cm{\pih_{t+1},x_{t+1}}\right]\label{Eqn:thm_follower6}- \epsilon_{t+1}\\
			&=\mE^{\sigma_t^f,\tsigma_{t}^l,\pi_t}\left[R^f(x_t,a_t) + \delta J^{f,\tsigma^f,\tsigma^l,\pih_{t+1}}_{t+1}\right]- \epsilon_{t+1}\label{Eqn:thm_follower7}\\
			&\geq\mE^{\sigma_t^f,\tsigma_{t}^l,\pi_t}[R^f(x_t,a_t) + \delta J^{f,\sigma_t^f,\tsigma_{t}^l,\pi_{t+1}}_{t+1}- \cm{1+\delta}\epsilon_{t+1}]\label{Eqn:thm_follower8}\\
			&=J^{f,\sigma_t^f,\tsigma_{t}^l,\pi_{t}}_{t} - \cm{1+\delta}\epsilon_{t+1}\label{Eqn:thm_follower9}
		\end{align}
		Thus, $J^{f,\tsigma^f,\tsigma^l,\pih_{t}}_{t} + \epsilon_{t}\geq J^{f,\sigma_t^f,\tsigma_{t}^l,\pi_{t}}_{t}$.

		~\eqref{Eqn:thm_follower2} is from Lemma~\ref{Lemma:V_optimal_returns2} and~\eqref{Eqn:thm_follower3} is from Lemma~\ref{Lemma:V_pf}.~\eqref{Eqn:thm_follower4} and~\eqref{Eqn:thm_follower5} are from standard definitions while ~\eqref{Eqn:thm_follower6} is true because ${V^\star}_{t+1}^l$ is optimal.~\eqref{Eqn:thm_follower7} is from Lemma~\ref{Lemma:V_optimal_returns2} followed by using assumption made at $t=t+1$ in~\eqref{Eqn:thm_follower8}.
	\end{proof}
\end{theorem}
\subsection{Convergence of the Leader}
We put forth two lemmas that is used to prove the theorems. The lemmas have not been proven in this section due to lack of space but could be referred from the online version.
\begin{lemma} 
	\label{Lemma:V_optimal_returns2}
	$\forall t\in\sq{T}$, $\forall \muh_t$,
	\begin{align}
		V_t^l\cm{\pih_t}= J^{l,\Lambda\cm{\tsigma^l},\tsigma^l,\pih}_t
	\end{align}
	where $\tsigma_t$ is the optimal policy at time $t$, $\pih_t = \muh_t[1:a_{1-1}]$ and $J_{t}$ is the accumulated optimal returns from $t$ till $T$.  
\end{lemma}

\begin{lemma} \label{Lemma:V_is_better2}
	$\forall t\in\cT$,$\forall \cm{a_{1:t-1}}\in\cH_t^f$,$\sigma_t^l$,
	\begin{align}
		\label{Eqn:lemma2_to_prove2}
		{V_t^\star}^l\left(\pi_t\right) \geq \mE^{\Lambda\cm{\sigma_t^l},\sigma_{t}^l,\pi_t}\left[{Q^\star}^l_{t}\left(\pi_t, A_t,\tgamma^f_{t}\right)\right]
	\end{align}
	where $\pi_t = \mu_t[1:a_{1-1}]$ and $V^\star$ and $Q^\star$ represent the value functions in the case where model is known.
\end{lemma}

\begin{theorem}\label{Thm:main_theorem1}
	A strategy $(\tilde{\sigma})$ constructed from the above algorithm is an $\epsilon$-\mpse of the game. i.e
	\begin{align}
		\label{Eqn:leader_main}
		J^{l,\tsigma^f,\tsigma^l,\pih_t}_t + \epsilon_t \geq J^{l,\Lambda\cm{\sigma^l},\sigma^l,\pi_t}_t
	\end{align}

	We prove it through the technique of mathematical induction and will use the results that were proved before in Lemma~\ref{Lemma:V_optimal_returns2} and Lemma~\ref{Lemma:V_is_better2}.

	\begin{proof}
	For the base case, we consider $t = T$. The expected sum of returns, when the player $i$ follows the equilibrium policy $\tsigma$ is given as
	\begin{align}
			J_T^{l,\Lambda\cm{\tsigma^l},\tsigma^l,\pi} = {V^\star}_T^l\left(\pi_T\right),\\
			J_T^{l,\Lambda\cm{\tsigma^l},\tsigma^l,\pih} = V_T^l\left(\pih_T\right),
		\end{align}
		which is true from Lemma~\ref{Lemma:V_optimal_returns2}.
	From Lemma~\ref{Lemma:V_pf}, 
	\begin{align}
		\label{Eqn:leader_thm1}
		{V^\star}_T^l\left(\pi_T\right) \leq  V_T^l\left(\pih_T\right) + \epsilon_T
	\end{align}
	for some chosen small $\epsilon_T$.
	
	
	From Lemma~\ref{Lemma:V_is_better2} and~\eqref{Eqn:leader_thm1} we get 
	\begin{align}
		J^{l,\tsigma^f,\tsigma^l,\pih_T}_T + \epsilon_T \geq J^{l,\Lambda\cm{\sigma^f},\tsigma^l,\pi_T}_T
	\end{align}
		Assuming that the condition in~\eqref{Eqn:leader_main} holds at $t = t+1$, we get,
		\begin{align}
			\label{Eqn:assumption2}
			J^{l,\tsigma^f,\tsigma^l,\pih_{t+1}}_{t+1} + \epsilon_{t+1} \geq J^{l,\Lambda\cm{\sigma^f},\tsigma^l,\pi_t}_{t+1}
		\end{align}
		We need to prove that the expression in~\eqref{Eqn:leader_main} holds for $t=t$ as well. 

		\begin{align}
			&J^{l,\tsigma^f,\tsigma^l,\pih_{t}}_{t}\label{Eqn:thm_leader1}\\
			&=V^l_t\cm{\pih_t}\label{Eqn:thm_leader2}\\
			&\geq{V^\star}^l_t\cm{\pi_t} - \epsilon_{t+1}\label{Eqn:thm_leader3}\\
			&\geq\mE^{\Lambda\cm{\sigma_t^l},\sigma_{t}^l,\pi_t}\left[{Q_t^\star}^l\left(\pi_t, x_t, A_t, \tgamma^f_{t}\right)\right]- \epsilon_{t+1}\label{Eqn:thm_leader4}\\
			&=\mE^{\Lambda\cm{\sigma_t^l},\sigma_{t}^l,\pi_t}\left[R^l(x_t,a_t) + \delta {V^\star}^l_{t+1}\cm{\pi_t}\right]- \epsilon_{t+1}\label{Eqn:thm_leader5}\\
			&\geq\mE^{\Lambda\cm{\sigma_t^l},\sigma_{t}^l,\pi_t}\left[R^l(x_t,a_t) + \delta {V}^l_{t+1}\cm{\pih_t}\right]\label{Eqn:thm_leader6}- \epsilon_{t+1}\\
			&=\mE^{\Lambda\cm{\sigma_t^l},\sigma_{t}^l,\pi_t}\left[R^l(x_t,a_t) + \delta J^{l,\tsigma^f,\tsigma^l,\pih_{t+1}}_{t+1}\right]- \epsilon_{t+1}\label{Eqn:thm_leader7}\\
			&\geq\mE^{\Lambda\cm{\sigma_t^l},\sigma_{t}^l,\pi_t}[R^l(x_t,a_t) + \delta J^{l,\Lambda\cm{\sigma^l},\sigma^l,\pi_{t+1}}_{t+1} \nn\\
			&- \cm{1+\delta}\epsilon_{t+1}]\label{Eqn:thm_leader8}\\
			&=J^{l,\Lambda\cm{\sigma^l},\sigma^l,\pi_{t}}_{t} - \cm{1+\delta}\epsilon_{t+1}\label{Eqn:thm_leader9}
		\end{align}
		Thus, $J^{l,\tsigma^f,\tsigma^l,\pih_{t}}_{t} + \epsilon_{t}\geq J^{l,\Lambda\cm{\sigma^l},\sigma^l,\pi_{t}}_{t}$.

		~\eqref{Eqn:thm_leader2} is from Lemma~\ref{Lemma:V_optimal_returns2} and~\eqref{Eqn:thm_leader3} is from Lemma~\ref{Lemma:V_pf}.~\eqref{Eqn:thm_leader4} and~\eqref{Eqn:thm_leader5} are from standard definitions while ~\eqref{Eqn:thm_leader6} is true because ${V^\star}_{t+1}^l$ is optimal.~\eqref{Eqn:thm_leader7} is from Lemma~\ref{Lemma:V_optimal_returns2} followed by using assumption made at $t=t+1$ in~\eqref{Eqn:thm_leader8}.
	\end{proof}


\end{theorem}

% 			 &=\mE^{\tsigma_t}\Bigg[R\cm{x_t^i,a_{t}^i,z_t} + \nn\\
% 			&\delta\mE^{\tsigma_{t+1:T}}\Bigg[\sum_{k = t+1}^T\delta^{k-t-1} R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t+1},x^i_{1:t+1}\Bigg]\Bigg]\label{Eqn:thm1_a}
% 		\end{align}
% 		Using Lemma~\ref{Lemma:V_optimal_returns}, and the definition of $V_t$ in~\eqref{Eqn:Vdef} we get,
% 		\begin{subequations}
% 			\begin{align}
% 				L=&\mE^{\tsigma_t}\sq{R\cm{x_t^i,a_{t}^i,z_t} + \delta V_{t+1}\cm{z_{1:t+1},x^i_{1:t+1}}}\\
% 				=&\mE^{\tsigma_t}\sq{Q_t\cm{z_t,x_t^i,a_t^i,\tsigma_t\cm{\cdot\vert z_t,\cdot}}}\\
% 				=&V_t\cm{z_t,x_t^i}
% 			\end{align}			
% 		\end{subequations}
% 		Now, from Lemma~\ref{Lemma:V_is_better},
% 		\begin{subequations}
% 			\begin{align}
% 				L\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t}, x_{t}^i, A_{t}^i,\tgamma_{t}} \vert z_t,x_t^i}\\
% 				=&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{R(z_t,x_t^i,a_t^i) + \delta V_{t+1}\cm{z_t,x_t^i}}\label{Eqn:Thm1_eqn6}
% 			\end{align}
% 		\end{subequations}
% 		which is true as per the definition in~\eqref{Eqn:Qdef}. The expression can now be expanded using Lemma~\ref{Lemma:V_optimal_returns} and use the assumption we made in~\eqref{Eqn:thm1_assumption}.
% 		\begin{subequations}
% 			\begin{align}
% 				L\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\Bigg[R(z_t,x_t^i,a_t^i) + \nn\\
% 				&\delta \mE^{\tsigma}\sq{\sum_{k=t}^{T}\delta^{k-t}R\left(x_k^i,A_k^i,z_k\right)\vert z_t,x_t^i}\Bigg]\\
% 				\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\Bigg[R(z_t,x_t^i,a_t^i) + \nn\\
% 				&\delta\mE^{\sigma^i\tsigma^{-i}}\sq{\sum_{k = t+1}^T\delta^{k-t- 1}R\cm{x_k^i,A_k^i,z_k}\big\vert z_{1:t+1},x^i_{1:t+1}}\Bigg]\\
% 				=&\mE^{\sigma^i,\tsigma^{-i}}\sq{\sum_{k = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,z_k}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\label{Eqn:Thm1_eqn10}
% 			\end{align}
% 		\end{subequations}
% 	\end{proof}
% \end{theorem}	
% \end{theorem}



% 	\begin{proof}
% 				Given that $\tsigma$ is the \mfe of the game, the equilibrium generating function such that
% 				\begin{align}
% 					\theta[z] = \tsigma\cm{\cdot\vert z,\cdot} \quad \forall z
% 				\end{align}
% 				At time $t$, let us assume that $\tgamma_t\cm{=\theta\sq{z_t}}$ be the prescription function that gives the equilibrium action but does not satisfy the fixed point equation in~\eqref{Eqn:fixed_point}, i.e.
% 				\begin{align}
% 					\tgamma_t\notin\arg\max_{\gamma_t}\mE^{\gamma_t}\sq{Q_t\cm{z_t,x_t^i, A_t^i,\tgamma_t}}
% 				\end{align}  
% 				Let us assume that $\hat{\gamma}_t$ be a solution to the fixed point equation in the \rl algorithm, then
% 				\begin{align}
% 					\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}
% 				\end{align}
% 				But, we know
% 				\begin{subequations}
% 					\begin{align}
% 						&\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 						&=\mE^{\hat{\sigma}_t}\sq{R_t\cm{z_t,x_t^i,A_t^i}+V_{t+1}\cm{z_{t+1},x^i_{t+1}}}\\
% 						&=\mE^{\hat{\sigma_t},\tsigma_{t+1:T}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\\
% 						&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 						&=V_t\cm{z_t,x_t^i}
% 					\end{align}
% 				\end{subequations}
% 				which is contradictory on the consideration that $\tsigma$ is a \mpe of the game.
% 			\end{proof}
% 		\end{theorem}	
		
% \end{theorem}	

% \begin{theorem}
% 	Let $\tilde{\sigma}$ be an \mfe of the mean-field game. Then there exists an equilibrium generating function $\theta$ that satisfies \eqref{Eqn:fixed_point} in the backward recursion algorithm such that $\tilde{\sigma}$ is defined using $\theta$.

% 	\begin{proof}
% 		Given that $\tsigma$ is the \mfe of the game, the equilibrium generating function such that
% 		\begin{align}
% 			\theta[z] = \tsigma\cm{\cdot\vert z,\cdot} \quad \forall z
% 		\end{align}
% 		At time $t$, let us assume that $\tgamma_t\cm{=\theta\sq{z_t}}$ be the prescription function that gives the equilibrium action but does not satisfy the fixed point equation in~\eqref{Eqn:fixed_point}, i.e.
% 		\begin{align}
% 			\tgamma_t\notin\arg\max_{\gamma_t}\mE^{\gamma_t}\sq{Q_t\cm{z_t,x_t^i, A_t^i,\tgamma_t}}
% 		\end{align}  
% 		Let us assume that $\hat{\gamma}_t$ be a solution to the fixed point equation in the \rl algorithm, then
% 		\begin{align}
% 			\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}
% 		\end{align}
% 		But, we know
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 				&=\mE^{\hat{\sigma}_t}\sq{R_t\cm{z_t,x_t^i,A_t^i}+V_{t+1}\cm{z_{t+1},x^i_{t+1}}}\\
% 				&=\mE^{\hat{\sigma_t},\tsigma_{t+1:T}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\\
% 				&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 				&=V_t\cm{z_t,x_t^i}
% 			\end{align}
% 		\end{subequations}
% 		which is contradictory on the consideration that $\tsigma$ is a \mpe of the game.
% 	\end{proof}
% \end{theorem}	

% \begin{assumption}
% 	\label{Assume:existence}
% 	Let the reward function $R\left(x_t^i, a_t^i, z_t\right)$ and the state transition matrix $\tau\left(x_{t+1}^i\vert x_t^i,a_t^i,z_t\right)$ be continuous functions in $z_t$.
% \end{assumption}	
% \begin{theorem}
% 	Under the assumption~\ref{Assume:existence}, there exists a solution to the fixed point equation in~\eqref{Eqn:fixed_point}.
% 	\begin{proof}
% 		It has already been shown that when the reward function is bounded, there exists a \mfe for finite horizon games. It can also been shown that the solutions to the fixed point equations are \mfe of the game. Thus there exists an equilibrium policy for the game achieved at each time $t$.
% 	\end{proof}
% \end{theorem}

% \subsection{Convergence for the leader}

% In this section, we prove the convergence of the proposed \rl algorithm to the equilibrium strategy of the statistical \mfg. Using backward recursion and sequential decomposition, the \rl algorithm is able to arrive at the equilibrium strategy for player $i$ at each time $t$. In other words, we show that the a player $i$ has no incentive to deviate from the equilibrium strategy $\tsigma$ given that the other players are playing the equilibrium strategy. Before proving convergence, we establish two lemmas related to the main theorems. In the first lemma we show that the action-value function $Q_t$ captures the expected sum of rewards accumulated by playing the $\tsigma$ at time $t$ by the $i^{th}$ player. We follow it with the proof of the next lemma establishing the optimality of the $Q$ value over the expected sum of rewards accumulated by playing any other strategy other than $\tsigma$. 

% \begin{lemma} 
% 	\label{Lemma:V_optimal_returns}
% 	$\forall t\in\sq{T}$, $\forall z_t$, $x_t^i\in\cX$,
% 	\begin{align}
% 		V_t\cm{z_t,x_t^i} &= \mE^{\tsigma_{t:T}}\left[\sum_{k=t}^{T}\delta^{k-t}R\left(x_k^i,A_k^i,z_k\right)\vert z_t,x_t^i\right]\\
% 		&=J_t
% 	\end{align}
% 	where $\tsigma_t$ is the optimal policy at time $t$ and $J_{t}$ is the accumulated optimal returns from $t$ till $T$. 
	

% 	\begin{proof}
% 		We prove the lemma using the theory of mathematical induction. 

% 		At $t=T$, from~\eqref{Eqn:Vdef},
% 		\begin{align}
% 			\label{Eqn:lemma1_eqn1}
% 			V_T\cm{z_T, x_T^i} =& \mE^{\tsigma_T}\sq{Q_T\cm{z_T, x_T^i, A_T^i, \tsigma_T\cm{\cdot\vert \cdot,z_t}}}\\
% 			=& \mE^{\tsigma_T}\sq{R\cm{z_T, x_T^i, A_T^i}},
% 		\end{align}
% 		which is true from~\eqref{Eqn:Qdef}. For any mean state $z_t$, $\tgamma_t=\tsigma_t\cm{\cdot\vert \cdot,z_t}$, therefore, we have,
% 		\begin{align}
% 			\label{Eqn:lemma_eqn2}
% 			V_T\cm{z_T,x_T^i} = \mE^{\tgamma_T}\sq{R\cm{x_T^i,A_T^i}}.
% 		\end{align}
% 		which is the maximum returns the agents can receive at $t=T$ because $\tgamma_t$ is the solution to the fixed point equation in~\eqref{Eqn:fixed_point} that maximizes~\eqref{Eqn:lemma_eqn2}.
		
% 		Now assuming that the proposition is true for $t = t+1$, we get,
% 		\begin{align} 	 
% 			&V_{t+1}\cm{z_{t+1},x_{t+1}^i} =J_{t+1}\\
% 			&=\mE^{\tsigma_{t+1:T}}\left[\sum_{k=t+1}^{T}\delta^{k-(t+1)}R\left(x_k^i,z_k\right)\vert z_{t+1},x_{t+1}^i\right]\label{Eqn:Lemma1_true_for_t+1}\\
% 		\end{align}
% 		At time $t = t$, we have,
% 		\begin{subequations}
% 			\begin{align}
% 				V_t\cm{z_t, x_t^i} = &\mE^{\tsigma_t}\sq{Q_t\cm{z_t, x_t^i, A_t^i, \tsigma_t\cm{\cdot\vert \cdot,z_t}}\vert z_t,x_t^i}\label{Eqn:Lemma1_eqn1}\\
% 								 = &\mE^{\tsigma_t}[R\cm{z_t, x_t^i, A_t^i}+\nn\\
% 								 &\delta V_{t+1}\cm{z_{t+1},x_{t+1}^i}\vert z_t,x_t^i]\label{Eqn:Lemma1_eqn2}
% 			\end{align}
% 		\end{subequations}
% 		\eqref{Eqn:Lemma1_eqn1} is from the definition in~\eqref{Eqn:Vdef} while~\eqref{Eqn:Lemma1_eqn2} is from the definition in~\eqref{Eqn:Qdef}. Using the assumption in~\eqref{Eqn:Lemma1_true_for_t+1}, we get,
% 		\begin{align}
% 			&V_t\cm{z_t, x_t^i} = \mE^{z_t, x_t^i}\Bigg[R\cm{z_t, x_t^i, A_t^i}+\nn\\
% 			&\delta  \mE^{\tsigma_{t+1:T}}\left[\sum_{k=t+1}^{T}\delta^{k-(t+1)}R\left(x_k^i,z_k\right)\vert z_{t+1},x_{t+1}^i\right]\Bigg]
% 		\end{align}
% 		Using the the expression for expected sum of returns in~\eqref{Eqn:j_func}, we get,
% 		\begin{align}
%             V_t\cm{z_t, x_t^i}    = \mE^{\tsigma_t}[R\cm{z_t, x_t^i, A_t^i}+\delta  J_{t+1}]
% 		\end{align}

% 	\end{proof}
% \end{lemma}

% \begin{lemma} \label{Lemma:V_is_better}
% 	$\forall i\in\cN$,$t\in\sq{T}$,$\forall z_t,x_t^i\in\cX,a^i_t\in\cA$,
% 	\begin{align}
% 		\label{Eqn:lemma2_to_prove}
% 		V_t\left(z_t,x_t^i\right) \geq \mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\left[Q_{t}\left(z_{t}, x_{t}^i, A_{t}^i,\tgamma_{t}\right) \vert z_t,x_t^i\right]
% 	\end{align}
% 	where $z_{t+1} = \phi\left(z_t,\tsigma_t\left(\cdot\vert z_t,\cdot\right)\right)$.


% 	\begin{proof}
% 		Given that at time $t+1$ the equilibrium policy is $\tsigma_{t+1}$ is the solution to the fixed point equation in~\eqref{Eqn:fixed_point}, let us assume that the player $i$ plays a different policy $\hat{\sigma}_{t+1}$ such that $\forall x^i_{t+1}\in\cX$,
% 		\begin{align}
% 			\label{Eqn:lemma2_not_in}
% 			\hat{\gamma}_{t}\cm{\cdot\vert x_{t+1}^i}\notin\arg\max_{\gamma_t} \mE\sq{Q_{t}\cm{z_{t},x_{t}^i,A_{t}^i,\tgamma_{t}} | z_{t},x_{t}^i}
% 		\end{align}
% 		with $\hat{\sigma}_{t}\cm{\cdot\vert z_{t},x_{t}^i}=\hat{\gamma}_{t}\cm{\cdot\vert x_{t}^i}$.

% 		Now, the equation on the other side of the inequality in\eqref{Eqn:lemma2_to_prove} can be changed assuming $\hat{\sigma}$ as the suboptimal policy as follows:
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t+1}, X_{t}^i,A_{t}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}\nn\\
% 				=&\mE^{\hat{\gamma}_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t}, x_{t}^i,A_{t}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}
% 			\end{align}
% 		\end{subequations}
% 		Considering~\eqref{Eqn:lemma2_not_in}, we can proceed as,
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\hat{\gamma}_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t}, X_{t}^i,A_{t}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}\nn\\
% 				\leq&\mE^{\tgamma_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t+1}, X_{t}^i,A_{t+1}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}\\
% 				=&V_t\left(z_t,x_t^i\right)
% 			\end{align}
% 		\end{subequations}
% 		where the last statement is from the definition in~\eqref{Eqn:Qdef}.
	
% 	\end{proof}
% \end{lemma}

% \begin{theorem}\label{Thm:main_theorem}
% 	A strategy $(\tilde{\sigma})$ constructed from the above algorithm is an \mfe of the game. i.e
% 	\begin{align}
% 		 &\mE^{\tsigma}\sq{\sum_{k = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t},x^i_{1:t}}\nn\\
% 		 &\geq\mE^{\sigma^i,\tsigma^{-i}}\sq{\sum_{k = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t},x^i_{1:t}}\label{Eqn:main_theorem}	
% 	\end{align}
% 	\begin{proof}
% 		We prove it through the technique of mathematical induction and will use the results that were proved before in Lemma~\ref{Lemma:V_optimal_returns} and Lemma~\ref{Lemma:V_is_better}.
		
% 		For the base case, we consider $t = T$. The expected sum of returns, when the player $i$ follows the equilibrium policy $\tsigma$ is given as
% 		\begin{align}
% 			J_T &= \mE^{\tsigma_T}\sq{R\cm{x_T^i,A_T^i,z_T}\big\vert z_{1:T},x^i_{1:T}}\\
% 				& = V_T\cm{z_T,x_T^i},
% 		\end{align}
% 		which is true from Lemma~\ref{Lemma:V_optimal_returns}.

% 		Now, from Lemma~\ref{Lemma:V_is_better}, we have,
% 			\begin{align}
% 				V_T\geq& \mE^{\sigma_{T}^i,\tsigma_{T}^{-i}}\left[Q_{T}\left(z_{T}, x_{T}^i, A_{T}^i,\tgamma_{T}\right) \vert z_t,x_t^i\right]\\
% 				=&\mE^{\sigma_T^i,\tsigma_T^{-i}}\sq{R\cm{x_T^i,A_T^i,z_T}\big\vert z_{1:T},x^i_{1:T}}
% 			\end{align}
% 		Assuming that the condition in~\eqref{Eqn:main_theorem} holds at $t = t+1$, we get,
% 		\begin{align}
% 			\begin{split}
% 				&\mE^{\tsigma}\sq{\sum_{k = t+1}^T\delta^{k-t-1}R\cm{x_k^i,A_k^i,z_k}\big\vert z_{1:t+1},x^i_{1:t+1}}\\
% 				&\geq\mE^{\sigma^i\tsigma^{-i}}\sq{\sum_{k = t+1}^T\delta^{k-t- 1}R\cm{x_k^i,A_k^i,z_k}\big\vert z_{1:t+1},x^i_{1:t+1}}\label{Eqn:thm1_assumption}
% 			\end{split}
% 		\end{align}
% 		We need to prove that the expression in~\eqref{Eqn:main_theorem} holds for $t=t$ as well. Let us represent the left hand side of~\eqref{Eqn:main_theorem} as $L$, i.e.
% 		\begin{align}
% 			\label{Eqn:thm1_t}
% 			L = \mE^{\tsigma}\sq{\sum_{n = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t},x^i_{1:t}}
% 		\end{align}
% 		The expectation at $t+1$ is independent of the rewards at time $t$, therefore, we can rewrite~\eqref{Eqn:thm1_t} as
% 		\begin{align}
% 			L &=\mE^{\tsigma_t}\Bigg[R\cm{x_t^i,a_{t}^i,z_t} + \nn\\
% 			&\delta\mE^{\tsigma_{t+1:T}}\Bigg[\sum_{k = t+1}^T\delta^{k-t-1} R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t+1},x^i_{1:t+1}\Bigg]\Bigg]\label{Eqn:thm1_a}
% 		\end{align}
% 		Using Lemma~\ref{Lemma:V_optimal_returns}, and the definition of $V_t$ in~\eqref{Eqn:Vdef} we get,
% 		\begin{subequations}
% 			\begin{align}
% 				L=&\mE^{\tsigma_t}\sq{R\cm{x_t^i,a_{t}^i,z_t} + \delta V_{t+1}\cm{z_{1:t+1},x^i_{1:t+1}}}\\
% 				=&\mE^{\tsigma_t}\sq{Q_t\cm{z_t,x_t^i,a_t^i,\tsigma_t\cm{\cdot\vert z_t,\cdot}}}\\
% 				=&V_t\cm{z_t,x_t^i}
% 			\end{align}			
% 		\end{subequations}
% 		Now, from Lemma~\ref{Lemma:V_is_better},
% 		\begin{subequations}
% 			\begin{align}
% 				L\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t}, x_{t}^i, A_{t}^i,\tgamma_{t}} \vert z_t,x_t^i}\\
% 				=&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{R(z_t,x_t^i,a_t^i) + \delta V_{t+1}\cm{z_t,x_t^i}}\label{Eqn:Thm1_eqn6}
% 			\end{align}
% 		\end{subequations}
% 		which is true as per the definition in~\eqref{Eqn:Qdef}. The expression can now be expanded using Lemma~\ref{Lemma:V_optimal_returns} and use the assumption we made in~\eqref{Eqn:thm1_assumption}.
% 		\begin{subequations}
% 			\begin{align}
% 				L\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\Bigg[R(z_t,x_t^i,a_t^i) + \nn\\
% 				&\delta \mE^{\tsigma}\sq{\sum_{k=t}^{T}\delta^{k-t}R\left(x_k^i,A_k^i,z_k\right)\vert z_t,x_t^i}\Bigg]\\
% 				\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\Bigg[R(z_t,x_t^i,a_t^i) + \nn\\
% 				&\delta\mE^{\sigma^i\tsigma^{-i}}\sq{\sum_{k = t+1}^T\delta^{k-t- 1}R\cm{x_k^i,A_k^i,z_k}\big\vert z_{1:t+1},x^i_{1:t+1}}\Bigg]\\
% 				=&\mE^{\sigma^i,\tsigma^{-i}}\sq{\sum_{k = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,z_k}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\label{Eqn:Thm1_eqn10}
% 			\end{align}
% 		\end{subequations}
% 	\end{proof}
% \end{theorem}	

% \begin{theorem}
% 	Let $\tilde{\sigma}$ be an \mfe of the mean field game. Then there exists an equilibrium generating function $\ttheta$ that satisfies \eqref{Eqn:fixed_point} in the backward recursion algorithm such that $\tilde{\sigma}$ is defined using $\ttheta$.

% 	\begin{proof}
% 		Given that $\tsigma$ is the \mfe of the game, the equilibrium generating function such that
% 		\begin{align}
% 			\ttheta[z] = \tsigma\cm{\cdot\vert z,\cdot} \quad \forall z
% 		\end{align}
% 		At time $t$, let us assume that $\tgamma_t\cm{=\ttheta\sq{z_t}}$ be the prescription function that gives the equilibrium action but does not satisfy the fixed point equation in~\eqref{Eqn:fixed_point}, i.e.
% 		\begin{align}
% 			\tgamma_t\notin\arg\max_{\gamma_t}\mE^{\gamma_t}\sq{Q_t\cm{z_t,x_t^i, A_t^i,\tgamma_t}}
% 		\end{align}  
% 		Let us assume that $\hat{\gamma}_t$ be a solution to the fixed point equation in the \rl algorithm, then
% 		\begin{align}
% 			\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}
% 		\end{align}
% 		But, we know
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 				&=\mE^{\hat{\sigma}_t}\sq{R_t\cm{z_t,x_t^i,A_t^i}+V_{t+1}\cm{z_{t+1},x^i_{t+1}}}\\
% 				&=\mE^{\hat{\sigma_t},\tsigma_{t+1:T}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\\
% 				&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 				&=V_t\cm{z_t,x_t^i}
% 			\end{align}
% 		\end{subequations}
% 		which is contradictory on the consideration that $\tsigma$ is a \mpe of the game.
% 	\end{proof}
% \end{theorem}	

% \begin{assumption}
% 	\label{Assume:existence}
% 	Let the reward function $R\left(x_t^i, a_t^i, z_t\right)$ and the state transition matrix $\tau\left(x_{t+1}^i\vert x_t^i,a_t^i,z_t\right)$ be continuous functions in $z_t$.
% \end{assumption}	
% \begin{theorem}
% 	Under the assumption~\ref{Assume:existence}, there exists a solution to the fixed point equation in~\eqref{Eqn:fixed_point}.
	
% 	\begin{proof}
% 		It has already been shown that when the reward function is bounded, there exists a \mfe for finite horizon games. It can also been shown that the solutions to the fixed point equations are \mfe of the game. Thus there exists an equilibrium policy for the game achieved at each time $t$.
% 	\end{proof}
% \end{theorem}
% In this section, we prove the convergence of the proposed \rl algorithm to the equilibrium strategy of the statistical \mfg. Using backward recursion and sequential decomposition, the \rl algorithm is able to arrive at the equilibrium strategy for player $i$ at each time $t$. In other words, we show that the a player $i$ has no incentive to deviate from the equilibrium strategy $\tsigma$ given that the other players are playing the equilibrium strategy. Before proving convergence, we establish two lemmas related to the main theorems. In the first lemma we show that the action-value function $Q_t$ captures the expected sum of rewards accumulated by playing the $\tsigma$ at time $t$ by the $i^{th}$ player. We follow it with the proof of the next lemma establishing the optimality of the $Q$ value over the expected sum of rewards accumulated by playing any other strategy other than $\tsigma$. 

% \begin{lemma} 
% 	\label{Lemma:V_optimal_returns}
% 	$\forall t\in\sq{T}$, $\forall z_t$, $x_t^i\in\cX$,
% 	\begin{align}
% 		V_t\cm{z_t,x_t^i} &= \mE^{\tsigma_{t:T}}\left[\sum_{k=t}^{T}\delta^{k-t}R\left(x_k^i,A_k^i,z_k\right)\vert z_t,x_t^i\right]\\
% 		&=J_t
% 	\end{align}
% 	where $\tsigma_t$ is the optimal policy at time $t$ and $J_{t}$ is the accumulated optimal returns from $t$ till $T$. 
	

% 	\begin{proof}
% 		We prove the lemma using the theory of mathematical induction. 

% 		At $t=T$, from~\eqref{Eqn:Vdef},
% 		\begin{align}
% 			\label{Eqn:lemma1_eqn1}
% 			V_T\cm{z_T, x_T^i} =& \mE^{\tsigma_T}\sq{Q_T\cm{z_T, x_T^i, A_T^i, \tsigma_T\cm{\cdot\vert \cdot,z_t}}}\\
% 			=& \mE^{\tsigma_T}\sq{R\cm{z_T, x_T^i, A_T^i}},
% 		\end{align}
% 		which is true from~\eqref{Eqn:Qdef}. For any mean state $z_t$, $\tgamma_t=\tsigma_t\cm{\cdot\vert \cdot,z_t}$, therefore, we have,
% 		\begin{align}
% 			\label{Eqn:lemma_eqn2}
% 			V_T\cm{z_T,x_T^i} = \mE^{\tgamma_T}\sq{R\cm{x_T^i,A_T^i}}.
% 		\end{align}
% 		which is the maximum returns the agents can receive at $t=T$ because $\tgamma_t$ is the solution to the fixed point equation in~\eqref{Eqn:fixed_point} that maximizes~\eqref{Eqn:lemma_eqn2}.
		
% 		Now assuming that the proposition is true for $t = t+1$, we get,
% 		\begin{align} 	 
% 			&V_{t+1}\cm{z_{t+1},x_{t+1}^i} =J_{t+1}\\
% 			&=\mE^{\tsigma_{t+1:T}}\left[\sum_{k=t+1}^{T}\delta^{k-(t+1)}R\left(x_k^i,z_k\right)\vert z_{t+1},x_{t+1}^i\right]\label{Eqn:Lemma1_true_for_t+1}\\
% 		\end{align}
% 		At time $t = t$, we have,
% 		\begin{subequations}
% 			\begin{align}
% 				V_t\cm{z_t, x_t^i} = &\mE^{\tsigma_t}\sq{Q_t\cm{z_t, x_t^i, A_t^i, \tsigma_t\cm{\cdot\vert \cdot,z_t}}\vert z_t,x_t^i}\label{Eqn:Lemma1_eqn1}\\
% 								 = &\mE^{\tsigma_t}[R\cm{z_t, x_t^i, A_t^i}+\nn\\
% 								 &\delta V_{t+1}\cm{z_{t+1},x_{t+1}^i}\vert z_t,x_t^i]\label{Eqn:Lemma1_eqn2}
% 			\end{align}
% 		\end{subequations}
% 		\eqref{Eqn:Lemma1_eqn1} is from the definition in~\eqref{Eqn:Vdef} while~\eqref{Eqn:Lemma1_eqn2} is from the definition in~\eqref{Eqn:Qdef}. Using the assumption in~\eqref{Eqn:Lemma1_true_for_t+1}, we get,
% 		\begin{align}
% 			&V_t\cm{z_t, x_t^i} = \mE^{z_t, x_t^i}\Bigg[R\cm{z_t, x_t^i, A_t^i}+\nn\\
% 			&\delta  \mE^{\tsigma_{t+1:T}}\left[\sum_{k=t+1}^{T}\delta^{k-(t+1)}R\left(x_k^i,z_k\right)\vert z_{t+1},x_{t+1}^i\right]\Bigg]
% 		\end{align}
% 		Using the the expression for expected sum of returns in~\eqref{Eqn:j_func}, we get,
% 		\begin{align}
%             V_t\cm{z_t, x_t^i}    = \mE^{\tsigma_t}[R\cm{z_t, x_t^i, A_t^i}+\delta  J_{t+1}]
% 		\end{align}

% 	\end{proof}
% \end{lemma}

% \begin{lemma} \label{Lemma:V_is_better}
% 	$\forall i\in\cN$,$t\in\sq{T}$,$\forall z_t,x_t^i\in\cX,a^i_t\in\cA$,
% 	\begin{align}
% 		\label{Eqn:lemma2_to_prove}
% 		V_t\left(z_t,x_t^i\right) \geq \mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\left[Q_{t}\left(z_{t}, x_{t}^i, A_{t}^i,\tgamma_{t}\right) \vert z_t,x_t^i\right]
% 	\end{align}
% 	where $z_{t+1} = \phi\left(z_t,\tsigma_t\left(\cdot\vert z_t,\cdot\right)\right)$.


% 	\begin{proof}
% 		Given that at time $t+1$ the equilibrium policy is $\tsigma_{t+1}$ is the solution to the fixed point equation in~\eqref{Eqn:fixed_point}, let us assume that the player $i$ plays a different policy $\hat{\sigma}_{t+1}$ such that $\forall x^i_{t+1}\in\cX$,
% 		\begin{align}
% 			\label{Eqn:lemma2_not_in}
% 			\hat{\gamma}_{t}\cm{\cdot\vert x_{t+1}^i}\notin\arg\max_{\gamma_t} \mE\sq{Q_{t}\cm{z_{t},x_{t}^i,A_{t}^i,\tgamma_{t}} | z_{t},x_{t}^i}
% 		\end{align}
% 		with $\hat{\sigma}_{t}\cm{\cdot\vert z_{t},x_{t}^i}=\hat{\gamma}_{t}\cm{\cdot\vert x_{t}^i}$.

% 		Now, the equation on the other side of the inequality in\eqref{Eqn:lemma2_to_prove} can be changed assuming $\hat{\sigma}$ as the suboptimal policy as follows:
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t+1}, X_{t}^i,A_{t}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}\nn\\
% 				=&\mE^{\hat{\gamma}_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t}, x_{t}^i,A_{t}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}
% 			\end{align}
% 		\end{subequations}
% 		Considering~\eqref{Eqn:lemma2_not_in}, we can proceed as,
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\hat{\gamma}_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t}, X_{t}^i,A_{t}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}\nn\\
% 				\leq&\mE^{\tgamma_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t+1}, X_{t}^i,A_{t+1}^i,\tgamma_{t}}\big\vert z_t,x_t^i,a_t^i}\\
% 				=&V_t\left(z_t,x_t^i\right)
% 			\end{align}
% 		\end{subequations}
% 		where the last statement is from the definition in~\eqref{Eqn:Qdef}.
	
% 	\end{proof}
% \end{lemma}

% \begin{theorem}\label{Thm:main_theorem}
% 	A strategy $(\tilde{\sigma})$ constructed from the above algorithm is an \mfe of the game. i.e
% 	\begin{align}
% 		 &\mE^{\tsigma}\sq{\sum_{k = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t},x^i_{1:t}}\nn\\
% 		 &\geq\mE^{\sigma^i,\tsigma^{-i}}\sq{\sum_{k = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t},x^i_{1:t}}\label{Eqn:main_theorem}	
% 	\end{align}
% 	\begin{proof}
% 		We prove it through the technique of mathematical induction and will use the results that were proved before in Lemma~\ref{Lemma:V_optimal_returns} and Lemma~\ref{Lemma:V_is_better}.
		
% 		For the base case, we consider $t = T$. The expected sum of returns, when the player $i$ follows the equilibrium policy $\tsigma$ is given as
% 		\begin{align}
% 			J_T &= \mE^{\tsigma_T}\sq{R\cm{x_T^i,A_T^i,z_T}\big\vert z_{1:T},x^i_{1:T}}\\
% 				& = V_T\cm{z_T,x_T^i},
% 		\end{align}
% 		which is true from Lemma~\ref{Lemma:V_optimal_returns}.

% 		Now, from Lemma~\ref{Lemma:V_is_better}, we have,
% 			\begin{align}
% 				V_T\geq& \mE^{\sigma_{T}^i,\tsigma_{T}^{-i}}\left[Q_{T}\left(z_{T}, x_{T}^i, A_{T}^i,\tgamma_{T}\right) \vert z_t,x_t^i\right]\\
% 				=&\mE^{\sigma_T^i,\tsigma_T^{-i}}\sq{R\cm{x_T^i,A_T^i,z_T}\big\vert z_{1:T},x^i_{1:T}}
% 			\end{align}
% 		Assuming that the condition in~\eqref{Eqn:main_theorem} holds at $t = t+1$, we get,
% 		\begin{align}
% 			\begin{split}
% 				&\mE^{\tsigma}\sq{\sum_{k = t+1}^T\delta^{k-t-1}R\cm{x_k^i,A_k^i,z_k}\big\vert z_{1:t+1},x^i_{1:t+1}}\\
% 				&\geq\mE^{\sigma^i\tsigma^{-i}}\sq{\sum_{k = t+1}^T\delta^{k-t- 1}R\cm{x_k^i,A_k^i,z_k}\big\vert z_{1:t+1},x^i_{1:t+1}}\label{Eqn:thm1_assumption}
% 			\end{split}
% 		\end{align}
% 		We need to prove that the expression in~\eqref{Eqn:main_theorem} holds for $t=t$ as well. Let us represent the left hand side of~\eqref{Eqn:main_theorem} as $L$, i.e.
% 		\begin{align}
% 			\label{Eqn:thm1_t}
% 			L = \mE^{\tsigma}\sq{\sum_{n = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t},x^i_{1:t}}
% 		\end{align}
% 		The expectation at $t+1$ is independent of the rewards at time $t$, therefore, we can rewrite~\eqref{Eqn:thm1_t} as
% 		\begin{align}
% 			L &=\mE^{\tsigma_t}\Bigg[R\cm{x_t^i,a_{t}^i,z_t} + \nn\\
% 			&\delta\mE^{\tsigma_{t+1:T}}\Bigg[\sum_{k = t+1}^T\delta^{k-t-1} R\cm{X_k^i,A_k^i,Z_k}\big\vert z_{1:t+1},x^i_{1:t+1}\Bigg]\Bigg]\label{Eqn:thm1_a}
% 		\end{align}
% 		Using Lemma~\ref{Lemma:V_optimal_returns}, and the definition of $V_t$ in~\eqref{Eqn:Vdef} we get,
% 		\begin{subequations}
% 			\begin{align}
% 				L=&\mE^{\tsigma_t}\sq{R\cm{x_t^i,a_{t}^i,z_t} + \delta V_{t+1}\cm{z_{1:t+1},x^i_{1:t+1}}}\\
% 				=&\mE^{\tsigma_t}\sq{Q_t\cm{z_t,x_t^i,a_t^i,\tsigma_t\cm{\cdot\vert z_t,\cdot}}}\\
% 				=&V_t\cm{z_t,x_t^i}
% 			\end{align}			
% 		\end{subequations}
% 		Now, from Lemma~\ref{Lemma:V_is_better},
% 		\begin{subequations}
% 			\begin{align}
% 				L\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{Q_{t}\cm{z_{t}, x_{t}^i, A_{t}^i,\tgamma_{t}} \vert z_t,x_t^i}\\
% 				=&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\sq{R(z_t,x_t^i,a_t^i) + \delta V_{t+1}\cm{z_t,x_t^i}}\label{Eqn:Thm1_eqn6}
% 			\end{align}
% 		\end{subequations}
% 		which is true as per the definition in~\eqref{Eqn:Qdef}. The expression can now be expanded using Lemma~\ref{Lemma:V_optimal_returns} and use the assumption we made in~\eqref{Eqn:thm1_assumption}.
% 		\begin{subequations}
% 			\begin{align}
% 				L\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\Bigg[R(z_t,x_t^i,a_t^i) + \nn\\
% 				&\delta \mE^{\tsigma}\sq{\sum_{k=t}^{T}\delta^{k-t}R\left(x_k^i,A_k^i,z_k\right)\vert z_t,x_t^i}\Bigg]\\
% 				\geq&\mE^{\sigma_{t}^i,\tsigma_{t}^{-i}}\Bigg[R(z_t,x_t^i,a_t^i) + \nn\\
% 				&\delta\mE^{\sigma^i\tsigma^{-i}}\sq{\sum_{k = t+1}^T\delta^{k-t- 1}R\cm{x_k^i,A_k^i,z_k}\big\vert z_{1:t+1},x^i_{1:t+1}}\Bigg]\\
% 				=&\mE^{\sigma^i,\tsigma^{-i}}\sq{\sum_{k = t}^T\delta^{k-t}R\cm{X_k^i,A_k^i,z_k}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\label{Eqn:Thm1_eqn10}
% 			\end{align}
% 		\end{subequations}
% 	\end{proof}
% \end{theorem}	

% \begin{theorem}
% 	Let $\tilde{\sigma}$ be an \mfe of the mean field game. Then there exists an equilibrium generating function $\ttheta$ that satisfies \eqref{Eqn:fixed_point} in the backward recursion algorithm such that $\tilde{\sigma}$ is defined using $\ttheta$.

% 	\begin{proof}
% 		Given that $\tsigma$ is the \mfe of the game, the equilibrium generating function such that
% 		\begin{align}
% 			\ttheta[z] = \tsigma\cm{\cdot\vert z,\cdot} \quad \forall z
% 		\end{align}
% 		At time $t$, let us assume that $\tgamma_t\cm{=\ttheta\sq{z_t}}$ be the prescription function that gives the equilibrium action but does not satisfy the fixed point equation in~\eqref{Eqn:fixed_point}, i.e.
% 		\begin{align}
% 			\tgamma_t\notin\arg\max_{\gamma_t}\mE^{\gamma_t}\sq{Q_t\cm{z_t,x_t^i, A_t^i,\tgamma_t}}
% 		\end{align}  
% 		Let us assume that $\hat{\gamma}_t$ be a solution to the fixed point equation in the \rl algorithm, then
% 		\begin{align}
% 			\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}
% 		\end{align}
% 		But, we know
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 				&=\mE^{\hat{\sigma}_t}\sq{R_t\cm{z_t,x_t^i,A_t^i}+V_{t+1}\cm{z_{t+1},x^i_{t+1}}}\\
% 				&=\mE^{\hat{\sigma_t},\tsigma_{t+1:T}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\\
% 				&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 				&=V_t\cm{z_t,x_t^i}
% 			\end{align}
% 		\end{subequations}
% 		which is contradictory on the consideration that $\tsigma$ is a \mpe of the game.
% 	\end{proof}
% \end{theorem}	

% \begin{assumption}
% 	\label{Assume:existence}
% 	Let the reward function $R\left(x_t^i, a_t^i, z_t\right)$ and the state transition matrix $\tau\left(x_{t+1}^i\vert x_t^i,a_t^i,z_t\right)$ be continuous functions in $z_t$.
% \end{assumption}	
% \begin{theorem}
% 	Under the assumption~\ref{Assume:existence}, there exists a solution to the fixed point equation in~\eqref{Eqn:fixed_point}.
	
% 	\begin{proof}
% 		It has already been shown that when the reward function is bounded, there exists a \mfe for finite horizon games. It can also been shown that the solutions to the fixed point equations are \mfe of the game. Thus there exists an equilibrium policy for the game achieved at each time $t$.
% 	\end{proof}
% \end{theorem}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{lemma}\label{Lemma:optimal_reward_is_Q} 
% 	The $Q$-value function computed by the player $i$ at time $t$ is same as the expected sum of rewards accrued by him by following the equilibrium policy $\tsigma = \cm{\tsigma_t}_t$ till time $T$, i.e. $\forall i\in\left[N\right]$,$t\in\sq{T}\backslash T$,$\cm{z_{1:t},x^i_{1:t},a^i_{1:t}}\in\cH_t^i$,
% 	\begin{align}
% 		\label{Eqn:lemma1_to_prove}
% 		Q_t\cm{z_t,x_t^i,a_t^i,\tsigma_t\cm{\cdot\vert z_t,\cdot}} = R(z_t,x_t^i,a^i_t)+ \nn\\
% 		\delta\mE^{\tsigma^i_{t+1:T},\tsigma^{-i}_{t+1:T}}\sq{\sum_{n = t+1}^T \delta^{n-t - 1}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_t,x_t^i,a_t^i}
% 	\end{align}
% 	where $z_{t+1} = \phi\cm{z_t,\tsigma_t\cm{\cdot\vert z_t,\cdot}}$ and $Q_T\cm{z_T,x_T,a_T,\cdot} = R\cm{x_T^i,a_T^i,z_T}$.		
% 	\begin{proof}
% 		We prove the lemma using the theory of mathematical induction. 
		
% 		At $t=T$, it is trivially true as per the definition in~\eqref{Eqn:lemma1_to_prove}. 
% 		For the base case, let us consider $t=T-1$. The expected sum of rewards is given as,
% 		\begin{align}
% 			\label{Eqn:lemma1_eqn1}
% 			R\cm{z_{T-1},x_{T-1}^i,a_{T-1}^i} + \delta\mE^{\tsigma^i_T,\tsigma^{-i}_T}\sq{R(X_T^i,A_{T}^i,z_T) | z_{T-1},x_{T-1}^i,a_{T-1}^i}.
% 		\end{align}
% 		Now the equation in~\eqref{Eqn:lemma1_eqn1} can be stated separately for each mean state $z_T$ such that $\tgamma_T=\tsigma\cm{\cdot\vert z_T,\cdot}$ as,
% 		\begin{subequations}
% 			\begin{align}
% 				&R\cm{z_{T-1},x_{T-1}^i,a_{T-1}^i} + \delta\mE^{\tgamma^i_T,\tsigma^{-i}_T}\sq{R(X_T^i,A_{T}^i,z_T^i) | z_{T-1},x_{T-1}^i,a_{T-1}^i}\nn\\
% 				=&R\cm{z_{T-1},x_{T-1}^i,a_{T-1}^i} + \delta\mE^{\tgamma^i_T,\tsigma^{-i}_T}\sq{Q_T\cm{x^i_T,a^i_T,z_T,\tgamma_T} | z_{T-1},x_{T-1}^i,a_{T-1}^i}\label{Eqn:lemma1_eqn2}\\
% 				=&Q_{T-1}\cm{x^i_{T-1},a^i_{T-1},z_{T-1},\tgamma_{T-1}}\label{Eqn:lemma1_eqn3}\\
% 				=&Q_{T-1}\cm{x^i_{T-1},a^i_{T-1},z_{T-1},\tsigma_{T-1}\cm{\cdot\vert z_{T-1},\cdot}}\label{Eqn:lemma1_eqn4}
% 			\end{align}
% 		\end{subequations}
% 		While~\eqref{Eqn:lemma1_eqn2} is true from the definition in~\eqref{Eqn:lemma1_to_prove}, the equations~\eqref{Eqn:lemma1_eqn3} and~\eqref{Eqn:lemma1_eqn4} follow from the algorithm definition in~\eqref{Eqn:Qdef}.


% 		Now assuming that the proposition is true for $t = t+1$, i.e.
% 		\begin{align}
% 			\begin{split}
% 				&Q_{t+1}\cm{z_{t+1},x_{t+1}^i,a_{t+1}^i,\tsigma_{t+1}\cm{\cdot\vert z_{t+1},\cdot}} =\\ 
% 				&R\cm{x_{t+1}^i,a_{t+1}^i,z_{t+1}} + \delta\mE^{\tsigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\sq{\sum_{n = t+2}^T \delta^{n-t-2}R\cm{X_n^i, A_n^i,Z_n} \Big\vert z_{t+1},x_{t+1}^i,a_{t+1}^i}
% 			\end{split}\label{Eqn:lemma1_true_for_t+1}
% 		\end{align}
		
% 		Then, at time $t = t$, the expected sum of discounted rewards is given as
% 		\begin{align}
% 			&R\cm{x_t^i,a^i_t,z_t} + \delta\mE^{\tsigma^i_{t+1:T},\tsigma^{-i}_{t+1:T}}\sq{\sum_{n = t+1}^T \delta^{n-t-1}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_t,x_t^i,a_t^i}
% 		\end{align}
% 		Segregating the rewards at time $t+1$ from the sum of rewards, we get,
% 		\begin{subequations}
% 			\begin{align}
% 				\begin{split}
% 					&R\cm{z_t,x_t^i,a_t^i}+\\
% 					&\delta\mE^{\tsigma^i_{t+1},\tsigma^{-i}_{t+1}}\sq{R\cm{X_{t+1}^i, A_{t+1}^i,Z_{t+1}} \big\vert z_t,x_t^i,a_t^i}+\\
% 					&\delta^2\mE^{\tsigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\sq{\sum_{n = t+2}^T \delta^{n-t-2}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_{t+1},x_{t+1}^i,a_{t+1}^i}
% 				\end{split}\nn\\
% 				\begin{split}
% 					=&R\cm{z_t,x_t^i,a_t^i}+\\
% 					&\delta\mE^{\tsigma^i_{t+1},\tsigma^{-i}_{t+1}}\Bigg[R\cm{X_{t+1}^i, A_{t+1}^i,Z_{t+1}} +\\
% 					&\delta\mE^{\tsigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\sq{\sum_{n = t+2}^T \delta^{n-t - 2}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_{t+1},x_{t+1}^i,a_{t+1}^i}\big\vert z_t,x_t^i,a_t^i\Bigg]
% 				\end{split}\label{Eqn:lemma1_eqn5}\\
% 				=&R\cm{z_t,x_t^i,a_t^i}+\delta\mE^{\tsigma^i_{t+1},\tsigma^{-i}_{t+1}}\sq{ Q_{t+1}\cm{z_{t+1},X_{t+1}^i,A_{t+1},\tsigma_{t+1}\cm{\cdot\vert z_{t+1},\cdot}}\big\vert z_{t},x_{t}^i,a_{t}^i}\label{Eqn:lemma1_eqn6}\\
% 				= &Q_{t}\cm{z_{t},x_{t}^i,a_{t},\tsigma_{t}\cm{\cdot\vert z_{t},\cdot}}\label{Eqn:lemma1_eqn7}
% 			\end{align}
% 		\end{subequations}
% 		\eqref{Eqn:lemma1_eqn5} is derived from the fact that expectation over a constant has no effect on the constant. Equation in~\eqref{Eqn:lemma1_eqn6} is true as per the assumption in \eqref{Eqn:lemma1_true_for_t+1} and~\eqref{Eqn:lemma1_eqn7} is from the definition in~\eqref{Eqn:Qdef}. 
	
% 	\end{proof}
% \end{lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this section, we prove that our proposed \rl algorithm converges to the stackelberg equilibrium for both the follower and the leader. The convergence of the sequential decomposition algorithm to the Stackelberg equilibrium was proved in~\cite{Vasal}. Here, we show that the estimated $Q-$values for the follower and the leader converge to the optimal $Q^\star$. We begin by stating the following Lemma: 
% \begin{lemma}
% 	\label{Lemma:main}
% 	Consider a stochastic process $\left(\alpha_t,\Delta_t,F_t\right)$ with $\alpha_t$, $\Delta_t$, $F_t:X\to\mathbb{R}$ which satisfies
% 	\begin{align}
% 	\label{eq:lemma_update}
% 	\Delta_{t+1}\left(x_t\right) = \left(1-\alpha_t\left(x_t\right)\right)\Delta_t\left(x_t\right) + \alpha_t\left(x_t\right)F_t\left(x_t\right)
% 	\end{align} 
% 	where $x_t\in X$ and $t = 0,1,2\ldots$. Let $\cF_t$ be a sequence of increasing $\sigma-$fields such that $\alpha_0$ and $\Delta_0$ are $\cF_0$-measurable and $\alpha_t$, $\Delta_t$ and $F_{t-1}$ are $\cF_t$-measurable, $t\geq1$. Assume that the following conditions hold:
% 	\begin{enumerate}
% 		\item $0<\alpha_t\left(x\right)<1$, $\sum{\alpha_t\left(x_t\right)}=\infty$, $\sum{\left(\alpha_t\left(x_t\right)\right)^2}<\infty$ w.p. $1$ and $\left\{\forall x\neq x_t: \alpha_t\left(x_t\right) = 0\right\}$
% 		\item $\lvert X\rvert<\infty$
% 		\item $\left\|\mE\left[F_t\vert\cF_t\right]\right\|\leq\kappa\lvert\lvert\Delta_t\rvert\rvert + C_t$ where $\kappa\in\left[0,1\right]$ and $C_t$ converges to $0$ w.p. $1$.
% 		\item Var$\left\{F_t\left(x_t\right)\vert\cF_t\right\}\leq K\left(1+\kappa\left\|\Delta_t\right\|\right)^2$ where $K$ is a constant. 
% 	\end{enumerate}
% 	where $\left\|..\right\|$ is denotes a maximum norm. Then $\Delta_t$ converges to $0$ w.p. $1$.
% \end{lemma}
% In the context of our model, let us introduce some straightforward assumptions that are essential to guarantee convergence.
% \begin{assumption}
% 	\label{asmp:assume1}
% 	State space $\cX$ and the action space $\cA$ are finite and each $(x_t,a_t^f, a_t^l)$ pairs is visited infinitely often.
% \end{assumption}
% \begin{assumption}
% 	\label{asmp:assume2}
% 	The policy is greedy in limit with infinite exploration.
% \end{assumption}
% \begin{assumption}
% 	\label{asmp:assume3}
% 	$0<\alpha_t\left(x_t^i\right)<1$, $\sum{\alpha_t\left(x_t^i\right)}=\infty$, $\sum{\left(\alpha_t\left(x_t^i\right)\right)^2}<\infty$ w.p. $1$ and $\left\{\forall x\neq x_t^i: \alpha_t\left(x\right) = 0\right\}$.
% \end{assumption}
% \begin{assumption}
% 	\label{asmp:assume4}
% 	The reward is bounded by some constant $K$.
% \end{assumption}

% \begin{theorem}
% 	\label{Th:value_func} In a finite-state stochastic Stackelberg game with asymmetric information between the leader and the follower, the functions $Q_t^f(\pi_t, x_t, a_t, \gamma_t^f)$ defined $\forall\pi_t\in\Pi$, $x_t\in\cX$, $a_t\in\cA$ and $Q_t^l(\pi_t, a_t^l, \gamma_t^f)$ defined $\forall\pi_t\in\Pi$, $a_t^l\in\cA^l$ estimated by the Algorithm~\ref{alg:Policy Evaluation} converges to the optimal values $Q^\star = \left(Q_t^f,Q_t^l\right)$ with policies $\tgammatf$ and $\tgammatl$ for each $\pi_t \in \Pi$ where $\theta\left[\pi_t\right]= \left(\tgammatf,\tgammatl\right)$ is an \mpse of the game.
% \end{theorem}

% We intend to use Lemma~\ref{Lemma:main} to prove theorem, i.e. we need to first show that with all the assumptions~\ref{asmp:assume1},\ref{asmp:assume2},\ref{asmp:assume3} and \ref{asmp:assume4}  being true, the conditions in  Lemma~\ref{Lemma:main} should also hold true. Then, by the statement of the lemma, we show convergence of the value function to $Q^\star$.  

% The Expected Sarsa update for the follower corresponding to any follower strategy $\tgammatf$ that is used in the algorithm can be rewritten as
% \begin{align}
% \label{eq:q_update}
% Q_t^f\left(\pi_t, x_t, a_t\right) = \left(1-\alpha\right)Q_t^f\left(\pi_t, x_t, a_t\right)+\nn\\ \alpha\left(R_t^f\left(x_t,a_t\right)+\delta V_{t+1}^f\left(\hat{\pi}_{t+1},x_{t+1}\right)\right)
% \end{align}
% where 
% \begin{align}
% V_{t+1}^f\left(x_{t+1},z_{t+1}\right) = \mE^{\tsigma_{t+1}^f,\tsigma_{t+1}^l}\left[Q_{t+1}^f\left(\hat{\pi}_{t+1},x_{t+1},A_{t+1}\right)\right]
% \end{align}
% We use $\hat{\pi}_{t+1}$ instead of $\pi_{t+1}$ as both the follower and the leader compute the value using separate particle filters which could give slightly different results. However, using law of large numbers, it can be shown that, in both cases, the values converge in expectation to the true value of the next belief state $\pi_{t+1}$. Thus, we need to show that
% \begin{align}
% \lim_{t\to\infty} Q_t^f\left(\pi_t, x_t, a_t\right) = Q^{\star,f}\left(\pi_t, x_t, a_t\right)
% \end{align}
% where 
% \begin{align}
% Q^{\star,f}\left(\pi_t, x_t, a_t\right) &= Q_t^f\left(\pi_t, x_t, a_t\right)\\
% &=\mE^{\tsigma_t}\left[R_t^f\left(\pi_t, x_t, a_t\right)+V^f_{t+1}\left(\pi_{t+1},X_{t+1}\right)\right]\nn\\
% &=\mE^{\tsigma_t}\left[R^f_t\left(\pi_t, x_t, a_t\right)+V^\star\left(\pi_{t+1},X_{t+1}\right)\right]\nn
% \end{align}
% where the expectation is over probability measure $Q_x\left(\cdot\vert x_t,a_t\right)$ for random variable $X_{t+1}$. In the subsequent discussions and proof we would drop all the obvious arguments except the time indices to make the equations more readable. Now, subtracting the optimal value function $Q^\star$ from~\eqref{eq:q_update}, and then comparing it with~\eqref{eq:lemma_update}, we get
% \begin{align}
% \label{eq:delt_ft}
% \Delta_t &= Q_t - Q^\star\\
%  \left\Vert\Delta_t\right\Vert&=\max_{\pi_ts_t,a_t}\lvert Q_t - Q^\star\rvert\\
% F_t &= R_t+\delta V_{t+1} - Q^\star\\
% &=R_t+\delta\mE^{\tsigma_{t}}\left[Q_t\right] -  Q^\star
% \end{align}
% We now proceed to the proof for Theorem~\ref{Th:value_func}.
% \begin{proof}
% 	Let us denote the $\sigma-$ fields generated by the trajectory $\left\{Q_0,x_0^i,a_0^i,r,x_1^i\ldots x_t^i\right\}$ by $\cF_t$. Since all the random variables in the trajectory till time instant $\tau<t$ are $\cF_t-$measurable, the functions $\Delta_t$ and $F_t$ are also $\cF_t-$measurable which satisfies the measurability condition of Lemma~\ref{Lemma:main}. Based on assumptions, it is straightforward to show that the first and the second condition of Lemma~\ref{Lemma:main} hold true.
	
% 	Let us now proceed to prove the condition $3$ and $4$ of Lemma~\ref{Lemma:main}. 
% 	We have,
% 	\begin{align}
% 	F_t &= R_t+\delta V_{t+1} - Q^\star\\
% 	&=R_t+\delta\mE^{\tsigma_{t}}\left[Q_t\right] -  Q^\star
% 	\end{align}
% 	$Q^\star$ is the optimal value that corresponds to the Stackelberg equilibrium. Let us define an operator $T:\mathcal{V}\to\mathcal{V}$ such that
% 	\begin{align}
% 	TQ_t = \mE\left[R_t + \delta V_t\right]
% 	\end{align}
% 	Now, 
% 	\begin{align}
% 	\left\|\mE\left[F_t\right\vert\cF_t]\right\| &= \left\|\mE\left[R_t+\delta V_{t+1}-Q^\star\right]\right\|\\
% 	&= \left\|\mE\left[R_t+\delta V_{t+1}-Q^\star + \max_{a_t}Q_t - \max_{a_t}Q_t\right]\right\|\nn\\
% 	&\leq \left\|\mE\left[\max_{a_t}Q_t-Q^\star ]\right]\right\| + \left\|\mE\left[R_t+\delta V_{t+1}- \max_{a_t}Q_t\right]\right\| \nn\\
% 	&\leq \left\|\max_{a_t}Q_t-Q^\star\right\| + \left\|\mE\left[\delta- \max_{a_t}Q_t\right]\right\| \nn\\
% 	&\leq \delta\left\|\Delta_t\right\| + C_t\nn
% 	\end{align}
% 	The third inequality is because of the fact that the policy derived by the fixed point equation forms a contraction mapping. $C_t = \left\|\mE\left[R_t+\delta V_t- Q_t\right]\right\|$ goes to $0$ w.p. $1$ as per the law of large numbers. This proves the third condition for Lemma~\ref{Lemma:main}. The 
% 	\begin{align}
% 	Var\left\{F_t\vert \cF_t\right\} &= \mE\left[\left(R_t+\delta V_t - Q_t^\star\right)^2\right]\\
% 	&= \mE\left[\left(R_t+\delta V_t - TQ_t^\star\right)^2\right]\\
% 	&= \mE\left[\left(R_t+\delta V_t - \mE\left[R_t + \delta V_t\right]\right)^2\right]\\
% 	&= Var\left\{R_t+\delta V_t\right\}\\
% 	&\leq K\left[1+{\left\|\Delta_t\right\|}^2\right]		 												 
% 	\end{align}
% 	The last inequality is a direct result of the Assumption~\ref{asmp:assume4}. This prove all the conditions of Lemma~\ref{Lemma:main} hold and thus we have
% 	\begin{align}
% 	\Delta_t&\to 0\\
% 	\text{i.e.}\quad Q_t&\to Q^\star
% 	\end{align}
% \end{proof}

% \begin{lemma}\label{Lemma:optimal_reward_is_Q} 
% 	The $Q$-value function computed by the player $i$ at time $t$ is same as the expected sum of rewards accrued by him by following the equilibrium policy $\tsigma = \cm{\tsigma_t}_t$ till time $T$, i.e. $\forall i\in\left[N\right]$,$t\in\sq{T}\backslash T$,$\cm{z_{1:t},x^i_{1:t},a^i_{1:t}}\in\cH_t^i$,
% 	\begin{align}
% 		\label{Eqn:lemma1_to_prove}
% 		Q_t\cm{z_t,x_t^i,a_t^i,\tsigma_t\cm{\cdot\vert z_t,\cdot}} = R(z_t,x_t^i,a^i_t) + \delta\mE^{\tsigma^i_{t+1:T},\tsigma^{-i}_{t+1:T}}\sq{\sum_{n = t+1}^T \delta^{n-t - 1}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_t,x_t^i,a_t^i}
% 	\end{align}
% 	where $z_{t+1} = \phi\cm{z_t,\tsigma_t\cm{\cdot\vert z_t,\cdot}}$ and $Q_T\cm{z_T,x_T,a_T,\cdot} = R\cm{x_T^i,a_T^i,z_T}$.		
% 	\begin{proof}
% 		We prove the lemma using the theory of mathematical induction. 
		
% 		At $t=T$, it is trivially true as per the definition in~\eqref{Eqn:lemma1_to_prove}. 
% 		For the base case, let us consider $t=T-1$. The expected sum of rewards is given as,
% 		\begin{align}
% 			\label{Eqn:lemma1_eqn1}
% 			R\cm{z_{T-1},x_{T-1}^i,a_{T-1}^i} + \delta\mE^{\tsigma^i_T,\tsigma^{-i}_T}\sq{R(X_T^i,A_{T}^i,z_T) | z_{T-1},x_{T-1}^i,a_{T-1}^i}.
% 		\end{align}
% 		Now the equation in~\eqref{Eqn:lemma1_eqn1} can be stated separately for each mean state $z_T$ such that $\tgamma_T=\tsigma\cm{\cdot\vert z_T,\cdot}$ as,
% 		\begin{subequations}
% 			\begin{align}
% 				&R\cm{z_{T-1},x_{T-1}^i,a_{T-1}^i} + \delta\mE^{\tgamma^i_T,\tsigma^{-i}_T}\sq{R(X_T^i,A_{T}^i,z_T^i) | z_{T-1},x_{T-1}^i,a_{T-1}^i}\nn\\
% 				=&R\cm{z_{T-1},x_{T-1}^i,a_{T-1}^i} + \delta\mE^{\tgamma^i_T,\tsigma^{-i}_T}\sq{Q_T\cm{x^i_T,a^i_T,z_T,\tgamma_T} | z_{T-1},x_{T-1}^i,a_{T-1}^i}\label{Eqn:lemma1_eqn2}\\
% 				=&Q_{T-1}\cm{x^i_{T-1},a^i_{T-1},z_{T-1},\tgamma_{T-1}}\label{Eqn:lemma1_eqn3}\\
% 				=&Q_{T-1}\cm{x^i_{T-1},a^i_{T-1},z_{T-1},\tsigma_{T-1}\cm{\cdot\vert z_{T-1},\cdot}}\label{Eqn:lemma1_eqn4}
% 			\end{align}
% 		\end{subequations}
% 		While~\eqref{Eqn:lemma1_eqn2} is true from the definition in~\eqref{Eqn:lemma1_to_prove}, the equations~\eqref{Eqn:lemma1_eqn3} and~\eqref{Eqn:lemma1_eqn4} follow from the algorithm definition in~\eqref{Eqn:Qdef}.


% 		Now assuming that the proposition is true for $t = t+1$, i.e.
% 		\begin{align}
% 			\begin{split}
% 				&Q_{t+1}\cm{z_{t+1},x_{t+1}^i,a_{t+1}^i,\tsigma_{t+1}\cm{\cdot\vert z_{t+1},\cdot}} =\\ 
% 				&R\cm{x_{t+1}^i,a_{t+1}^i,z_{t+1}} + \delta\mE^{\tsigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\sq{\sum_{n = t+2}^T \delta^{n-t-2}R\cm{X_n^i, A_n^i,Z_n} \Big\vert z_{t+1},x_{t+1}^i,a_{t+1}^i}
% 			\end{split}\label{Eqn:lemma1_true_for_t+1}
% 		\end{align}
		
% 		Then, at time $t = t$, the expected sum of discounted rewards is given as
% 		\begin{align}
% 			&R\cm{x_t^i,a^i_t,z_t} + \delta\mE^{\tsigma^i_{t+1:T},\tsigma^{-i}_{t+1:T}}\sq{\sum_{n = t+1}^T \delta^{n-t-1}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_t,x_t^i,a_t^i}
% 		\end{align}
% 		Segregating the rewards at time $t+1$ from the sum of rewards, we get,
% 		\begin{subequations}
% 			\begin{align}
% 				\begin{split}
% 					&R\cm{z_t,x_t^i,a_t^i}+\\
% 					&\delta\mE^{\tsigma^i_{t+1},\tsigma^{-i}_{t+1}}\sq{R\cm{X_{t+1}^i, A_{t+1}^i,Z_{t+1}} \big\vert z_t,x_t^i,a_t^i}+\\
% 					&\delta^2\mE^{\tsigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\sq{\sum_{n = t+2}^T \delta^{n-t-2}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_{t+1},x_{t+1}^i,a_{t+1}^i}
% 				\end{split}\nn\\
% 				\begin{split}
% 					=&R\cm{z_t,x_t^i,a_t^i}+\\
% 					&\delta\mE^{\tsigma^i_{t+1},\tsigma^{-i}_{t+1}}\Bigg[R\cm{X_{t+1}^i, A_{t+1}^i,Z_{t+1}} +\\
% 					&\delta\mE^{\tsigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\sq{\sum_{n = t+2}^T \delta^{n-t - 2}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_{t+1},x_{t+1}^i,a_{t+1}^i}\big\vert z_t,x_t^i,a_t^i\Bigg]
% 				\end{split}\label{Eqn:lemma1_eqn5}\\
% 				=&R\cm{z_t,x_t^i,a_t^i}+\delta\mE^{\tsigma^i_{t+1},\tsigma^{-i}_{t+1}}\sq{ Q_{t+1}\cm{z_{t+1},X_{t+1}^i,A_{t+1},\tsigma_{t+1}\cm{\cdot\vert z_{t+1},\cdot}}\big\vert z_{t},x_{t}^i,a_{t}^i}\label{Eqn:lemma1_eqn6}\\
% 				= &Q_{t}\cm{z_{t},x_{t}^i,a_{t},\tsigma_{t}\cm{\cdot\vert z_{t},\cdot}}\label{Eqn:lemma1_eqn7}
% 			\end{align}
% 		\end{subequations}
% 		\eqref{Eqn:lemma1_eqn5} is derived from the fact that expectation over a constant has no effect on the constant. Equation in~\eqref{Eqn:lemma1_eqn6} is true as per the assumption in \eqref{Eqn:lemma1_true_for_t+1} and~\eqref{Eqn:lemma1_eqn7} is from the definition in~\eqref{Eqn:Qdef}. 
	
% 	\end{proof}
% \end{lemma}

% \begin{lemma} \label{Lemma:Q_is_better}
% 	$\forall i\in\left[N\right]$,$t\in\sq{T}$,$\forall z_t,x_t^i\in\cX,a^i_t\in\cA$,
% 	\begin{align}
% 		\label{Eqn:lemma2_to_prove}
% 		Q_t\left(z_t,x_t^i,a_t^i,\tsigma_t\left(\cdot\vert z_t,\cdot\right)\right) \geq R(x_t^i,a_t^i,z_t) + \delta\mE^{\sigma_{t+1}^i,\tsigma_{t+1}^{-i}}\left[Q_{t+1}(z_{t+1}, X_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}) | z_t,x_t^i\right]
% 	\end{align}
% 	where $z_{t+1} = \phi\left(z_t,\tsigma_t\left(\cdot\vert z_t,\cdot\right)\right)$ and $\tgamma_{t+1}=\tsigma_{t+1}\cm{\cdot\vert z_{t+1},\cdot}$
% 	\begin{proof}
% 		Given that at time $t+1$ the equilibrium policy is $\tsigma_{t+1}$ is the solution to the fixed point equation in~\eqref{Eqn:fixed_point}, let us assume that the player $i$ plays a different policy $\hat{\sigma}_{t+1}$ such that $\forall x^i_{t+1}\in\cX$,
% 		\begin{align}
% 			\label{Eqn:lemma2_not_in}
% 			\hat{\gamma}_{t+1}\cm{\cdot\vert x_{t+1}^i}\notin\arg\max_{\gamma_{t+1}} \mE\sq{Q_{t+1}\cm{z_{t+1},x_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}} | z_{t+1},x_{t+1}^i}
% 		\end{align}
% 		with $\hat{\sigma}_{t+1}\cm{\cdot\vert z_{t+1},x_{t+1}^i}=\hat{\gamma}_{t+1}\cm{\cdot\vert x_{t+1}^i}$.

% 		Now, the equation on the other side of the inequality in\eqref{Eqn:lemma2_to_prove} can be changed assuming $\hat{\sigma}$ as the suboptimal policy as follows:
% 		\begin{subequations}
% 			\begin{align}
% 				&R(z_t,x_t^i,a_t^i) + \delta\mE^{\sigma_{t+1}^i,\tsigma_{t+1}^{-i}}\sq{Q_{t+1}\cm{z_{t+1}, X_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}}\big\vert z_t,x_t^i,a_t^i}\nn\\
% 				=&R(z_t,x_t^i,a_t^i) + \delta\mE^{\hat{\gamma}_{t+1}^i,\tsigma_{t+1}^{-i}}\sq{Q_{t+1}\cm{z_{t+1}, X_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}}\big\vert z_t,x_t^i,a_t^i}
% 			\end{align}
% 		\end{subequations}
% 		Considering~\eqref{Eqn:lemma2_not_in}, we can proceed as,
% 		\begin{subequations}
% 			\begin{align}
% 				&R(z_t,x_t^i,a_t^i) + \delta\mE^{\hat{\gamma}_{t+1}^i,\tsigma_{t+1}^{-i}}\sq{Q_{t+1}\cm{z_{t+1}, X_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}}\big\vert z_t,x_t^i,a_t^i}\nn\\
% 				\leq&R(z_t,x_t^i,a_t^i) + \delta\mE^{\tgamma_{t+1}^i,\tsigma_{t+1}^{-i}}\sq{Q_{t+1}\cm{z_{t+1}, X_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}}\big\vert z_t,x_t^i,a_t^i}\\
% 				=&Q_t\left(z_t,x_t^i,a_t,\tsigma_t\left(\cdot\vert z_t,\cdot\right)\right)
% 			\end{align}
% 		\end{subequations}
% 		where the last statement is from the definition in~\eqref{Eqn:Qdef}.
	
% 	\end{proof}
% \end{lemma}

% \begin{theorem}\label{Thm:main_theorem}
% 	A strategy $(\tilde{\sigma})$ constructed from the above algorithm is an \mfe of the game. i.e
% 	\begin{align}
% 		\label{Eqn:main_thorem}
% 		 \mE^{\tsigma}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\geq\mE^{\sigma^i,\tsigma^{-i}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}
% 	\end{align}
% 	\begin{proof}
% 		We prove it through the technique of mathematical induction and will use the results that were proved before in Lemma~\ref{Lemma:optimal_reward_is_Q} and Lemma~\ref{Lemma:Q_is_better}.
		
% 		For the base case, we consider $t = T-1$ as $t=T$ is a trivial case. The expected sum of returns, when the player $i$ follows the equilibrium policy $\tsigma$ is given as
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\tsigma}\sq{\sum_{n = T-1}^T\delta^{n-T-1}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:T-1},x^i_{1:T-1},a_{1:T-1}^i}\nn\\
% 				=&R\cm{x_{T-1}^i,a_{T-1}^i,z_{T-1}} + \delta\mE^{\tsigma_T}\sq{\sum_{n = T}^T\delta^{n-T} R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:T-1},x^i_{1:T-1},a_{1:T-1}^i}\label{Eqn:Thm1_eqn1}\\
% 				=&Q_T\cm{Z_{T-1}X_{T-1}^i,A_{T-1}^i}\label{Eqn:Thm1_eqn2}\\
% 				\geq &R\cm{X_{T-1}^i,A_{T-1}^i,Z_{T-1}} + \delta\mE^{\sigma_T^i,\tsigma_T^{-i}}\sq{\sum_{n = T}^T\delta^{n-T} R\cm{X_T^i,A_T^i,Z_n}\big\vert z_{1:T-1},x^i_{1:T-1},a_{1:T-1}^i}\label{Eqn:Thm1_eqn3}\\
% 				=&\mE^{\sigma_T^i,\tsigma_T^{-i}}\sq{\sum_{n = T-1}^T\delta^{n-T + 1}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\label{Eqn:Thm1_eqn4} 
% 			\end{align}
% 		\end{subequations}
% 		where~\eqref{Eqn:Thm1_eqn1} follows from the derivation in Lemma~\ref{Lemma:optimal_reward_is_Q} while~\eqref{Eqn:Thm1_eqn4} follows from Lemma~\ref{Lemma:Q_is_better}.

% 		Now, assuming that the condition in~\eqref{Eqn:main_thorem} holds at $t = t+1$, we get,
% 		\begin{align}
% 			\begin{split}
% 				\mE^{\tsigma}&\sq{\sum_{n = t+1}^T\delta^{n-t-1}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t+1},x^i_{1:t+1},a_{1:t+1}^i}\\
% 				&\geq\mE^{\sigma}\sq{\sum_{n = t+1}^T\delta^{n-t- 1}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t+1},x^i_{1:t+1},a_{1:t+1}^i}
% 			\end{split}
% 		\end{align}
% 		We need to prove that the expression in~\eqref{Eqn:main_thorem} holds for $t=t$ as well.
% 		\begin{subequations}
% 			\begin{align}
% 				&\mE^{\tsigma}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\nn\\
% 				=&R\cm{x_t^i,a_{t}^i,z_t} + \delta\mE^{\tsigma_{t+1:T}}\sq{\sum_{n = t+1}^T\delta^{n-t-1} R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\nn\\
% 				=&Q_t\cm{z_t,x_t^i,a_t^i,\tsigma_t\cm{\cdot\vert z_t,\cdot}}\label{Eqn:Thm1_eqn5}\\
% 				\geq &R(z_t,x_t^i,a_t^i) + \delta\mE^{\sigma_{t+1}^i,\tsigma_{t+1}^{-i}}\sq{Q_{t+1}\cm{z_{t+1}, X_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}} | z_t,x_t^i}\label{Eqn:Thm1_eqn6}\\
% 				\begin{split}
% 					=&R(z_t,x_t^i,a_t^i) + \delta\mE^{\sigma_{t+1}^i,\tsigma_{t+1}^{-i}}\Bigg[R(z_{t+1},x_{t+1}^i,a^i_{t+1}) + \\
% 					&\delta\mE^{\tsigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\Bigg[\sum_{n = t+2}^T \delta^{n-t-2}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_t,x_t^i,a_t^i\Bigg]\Bigg]
% 				\end{split}\label{Eqn:Thm1_eqn7}\\
% 				\begin{split}
% 					\geq&R(z_t,x_t^i,a_t^i) + \delta\mE^{\sigma_{t+1}^i,\tsigma_{t+1}^{-i}}\Bigg[R(z_{t+1},x_{t+1}^i,a^i_{t+1}) + \\
% 					&\delta\mE^{\sigma^i_{t+2:T},\tsigma^{-i}_{t+2:T}}\Bigg[\sum_{n = t+2}^T \delta^{n-t-2}R\cm{X_n^i, A_n^i,Z_n} \big\vert z_t,x_t^i,a_t^i\Bigg]\Bigg]
% 				\end{split}\label{Eqn:Thm1_eqn8}\\
% 				=&R\cm{x_t^i,a_{t}^i,z_t} + \mE^{\sigma^i_{t+1:T},\tsigma^{-i}_{t+1:T}}\sq{\sum_{n = t+1}^T\delta^{n-t} R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\label{Eqn:Thm1_eqn9}\\
% 				=&\mE^{\sigma^i,\tsigma^{-i}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\label{Eqn:Thm1_eqn10}
% 			\end{align}
% 		\end{subequations}

% 		\eqref{Eqn:Thm1_eqn5} and~\eqref{Eqn:Thm1_eqn6} follow from the Lemmas~\ref{Lemma:optimal_reward_is_Q} and~\ref{Lemma:Q_is_better} respectively. Again, we use Lemma~\ref{Lemma:optimal_reward_is_Q} to substitute for $Q_{t+1}$ to get~\eqref{Eqn:Thm1_eqn7}. This decomposition could be repeated till $T$ to get~\eqref{Eqn:Thm1_eqn8} and~\eqref{Eqn:Thm1_eqn9} and~\eqref{Eqn:Thm1_eqn10} follow accordingly.

% 	\end{proof}
% \end{theorem}	

% \begin{theorem}
% 	Let $\tilde{\sigma}$ be an \mfe of the mean field game. Then there exists an equilibrium generating function $\theta$ that satisfies \eqref{Eqn:fixed_point} in the backward recursion algorithm such that $\tilde{\sigma}$ is defined using $\theta$.

% 	\begin{proof}
% 		Given that $\tsigma$ is the \mfe of the game, the equilibrium generating function such that
% 		\begin{align}
% 			\theta[z] = \tsigma\cm{\cdot\vert z,\cdot} \quad \forall z
% 		\end{align}
% 		At time $t$, let us assume that $\tgamma_t\cm{=\theta\sq{z_t}}$ be the prescription function that gives the equilibrium action but does not satisfy the fixed point equation in~\eqref{Eqn:fixed_point}, i.e.
% 		\begin{align}
% 			\tgamma_t\notin\arg\max_{\gamma_t}\mE^{\gamma_t}\sq{Q_t\cm{z_t,x_t^i, A_t^i,\tgamma_t}}
% 		\end{align}  
% 		Let us assume that $\hat{\gamma}_t$ be a solution to the fixed point equation in the \rl algorithm, then
% 		\begin{align}
% 			\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}
% 		\end{align}
% 		But, we know
% 		\begin{subequations}
% 			\begin{align}
% 				\mE^{\hat{\gamma}_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}&=\mE^{\hat{\sigma}_t}\sq{R_t\cm{z_t,x_t^i,A_t^i}+\mE^{\tsigma_{t+1}}\sq{Q_{t+1}\cm{z_{t+1},x_{t+1}^i,A_{t+1}^i,\tgamma_{t+1}}}}\\
% 				&=\mE^{\hat{\sigma_t},\tsigma_{t+1:T}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}\\
% 				&\geq\mE^{\tgamma_t}\sq{Q_t\cm{z_t,x_t^i,A_t^i,\tgamma_t}}\\
% 				&=\mE^{\tsigma_t,\tsigma_{t+1:T}}\sq{\sum_{n = t}^T\delta^{n-t}R\cm{X_n^i,A_n^i,Z_n}\big\vert z_{1:t},x^i_{1:t},a_{1:t}^i}
% 			\end{align}
% 		\end{subequations}
% 		which is contradictory on the consideration that $\tsigma$ is a \mpe of the game.
% 	\end{proof}
% \end{theorem}	

% \begin{assumption}
% 	\label{Assume:existence}
% 	Let the reward function $R\left(x_t^i, a_t^i, z_t\right)$ and the state transition matrix $\tau\left(x_{t+1}^i\vert x_t^i,a_t^i,z_t\right)$ be continuous functions in $z_t$.
% \end{assumption}	
% \begin{theorem}
% 	Under the assumption~\ref{Assume:existence}, there exists a solution to the fixed point equation in~\eqref{Eqn:fixed_point}.
% 	\begin{proof}
% 		It has already been shown that when the reward function is bounded, there exists a \mfe for finite horizon games. It can also been shown that the solutions to the fixed point equations are \mfe of the game. Thus there exists an equilibrium policy for the game achieved at each time $t$.
% 	\end{proof}
% \end{theorem}

% \begin{lemma}
% 	\label{Lemma:main}
% 	Consider a stochastic process $\left(\alpha_t,\Delta_t,F_t\right)$ with $\alpha_t$, $\Delta_t$, $F_t:X\to\mathbb{R}$ which satisfies
% 	\begin{align}
% 	\label{eq:lemma_update}
% 	\Delta_{t+1}\left(x_t\right) = \left(1-\alpha_t\left(x_t\right)\right)\Delta_t\left(x_t\right) + \alpha_t\left(x_t\right)F_t\left(x_t\right)
% 	\end{align} 
% 	where $x_t\in X$ and $t = 0,1,2\ldots$. Let $\cF_t$ be a sequence of increasing $\sigma-$fields such that $\alpha_0$ and $\Delta_0$ are $\cF_0$-measurable and $\alpha_t$, $\Delta_t$ and $F_{t-1}$ are $\cF_t$-measurable, $t\geq1$. Assume that the following conditions hold:
% 	\begin{enumerate}
% 		\item $0<\alpha_t\left(x\right)<1$, $\sum{\alpha_t\left(x_t\right)}=\infty$, $\sum{\left(\alpha_t\left(x_t\right)\right)^2}<\infty$ w.p. $1$ and $\left\{\forall x\neq x_t: \alpha_t\left(x_t\right) = 0\right\}$
% 		\item $\lvert X\rvert<\infty$
% 		\item $\left\|\mE\left[F_t\vert\cF_t\right]\right\|\leq\kappa\lvert\lvert\Delta_t\rvert\rvert + C_t$ where $\kappa\in\left[0,1\right]$ and $C_t$ converges to $0$ w.p. $1$.
% 		\item Var$\left\{F_t\left(x_t\right)\vert\cF_t\right\}\leq K\left(1+\kappa\left\|\Delta_t\right\|\right)^2$ where $K$ is a constant. 
% 	\end{enumerate}
% where $\left\|..\right\|$ is denotes a maximum norm. Then $\Delta_t$ converges to $0$ w.p. $1$.
% \end{lemma}
% In the context of our model, let us introduce some straightforward assumptions that are essential to guarantee convergence.
% \begin{assumption}
% 	\label{asmp:assume1}
% 	State space $\cX$ and the action space $\cA$ are finite and each $(x_t^i,a_t^i)$ pairs is visited infinitely often.
% \end{assumption}
% \begin{assumption}
% 	\label{asmp:assume2}
% 	 The policy is greedy in limit with infinite exploration (GLIE).
% \end{assumption}
% \begin{assumption}
% 	\label{asmp:assume3}
% 	$0<\alpha_t\left(x_t^i\right)<1$, $\sum{\alpha_t\left(x_t^i\right)}=\infty$, $\sum{\left(\alpha_t\left(x_t^i\right)\right)^2}<\infty$ w.p. $1$ and $\left\{\forall x\neq x_t^i: \alpha_t\left(x\right) = 0\right\}$.
% \end{assumption}
% \begin{assumption}
% 	\label{asmp:assume4}
% 	The reward is bounded by some constant $K$.
% \end{assumption}

% \begin{theorem}
% 	\label{Th:value_func} In a finite-state stochastic game, the $Q_t^{\tsigma_{t}}$ values estimated by the algorithm~\ref{alg:Evaluation} converges to the optimal values $Q^\star = Q_t^{\tsigma}\left(x_t^i,a_t^i,z_t\right)$ for each $z_t \in \cZ$ where $\tsigma$ is an \mpe of the game.
% \end{theorem}
% The theorem for convergence have been proved in a similar way in~\cite{Yang2018} for \mfe in multi-agent \rl setting but with average action as the common information. We intend to use Lemma~\ref{Lemma:main} to prove theorem, i.e. we need to first show that with all the assumptions~\ref{asmp:assume1},\ref{asmp:assume2},\ref{asmp:assume3} and \ref{asmp:assume4}  being true, the conditions in  Lemma~\ref{Lemma:main} should also hold true. Then, by the statement of the lemma, we show convergence of the value function to $Q^\star$.  
 
% The expected sarsa update that is used in the algorithm can be rewritten as
% \begin{align}
% 	\label{eq:q_update}
% 	Q_t^{\sigma_t}\left(x_t^i,a_t^i,z_t\right) = \left(1-\alpha\right)Q_t^{\sigma_t}\left(x_t^i,a_t^i,z_t\right) +\nn\\ \alpha\left(R_t\left(x_t^i,a_t^i,z_t\right)+\delta V_{t+1}^{\sigma_{t}}\left(x_{t+1},z_{t+1}\right)\right)
% \end{align}
% where 
% \begin{align}
% 	V_{t+1}^{\sigma_{t}}\left(x_{t+1},z_{t+1}\right) = \mE^{\sigma_{t}}\left[Q_{t+1}^{\sigma_{t}}\left(x_{t+1}^i,A_{t+1}^i,z_{t+1}\right)\right]
% \end{align}
% Basically, our aim is to show that
% \begin{align}
% 	\lim_{t\to\infty} Q_t^{\sigma_t}\left(x_t^i,a_t^i,z_t\right) = Q^\star\left(x_t^i,a_t^i,z_t\right)
% \end{align}
% where 
% \begin{align}
% Q^\star\left(x_t^i,a_t^i,z_t\right) &= Q^{\tsigma_t}\left(x_t^i,a_t^i,z_t\right)\\
% &=\mE\left[R_t\left(x_t^i,a_t^i,z_t\right)+V^{\tsigma}\left(X_{t+1},z_{t+1}\right)\right]\nn\\
% &=\mE\left[R_t\left(x_t^i,a_t^i,z_t\right)+V^\star\left(X_{t+1},z_{t+1}\right)\right]\nn
% \end{align}
% where the expectation is over probability measure $Q_x\left(\cdot\vert x_t^i,a_t^i\right)$ for random variable $X_{t+1}^i$.


% In the subsequent discussions and proof we would drop all the obvious arguments except the time indices to make the equations more readable. Now, subtracting the optimal value function $Q^\star$ from~\eqref{eq:q_update}, and then comparing it with~\eqref{eq:lemma_update}, we get
% \begin{align}
% 	\label{eq:delt_ft}
%  	\Delta_t &= Q_t - Q^\star\\
%  	F_t &= R_t+\delta V_{t+1} - Q^\star
% \end{align}
% We now proceed to the proof for Theorem~\ref{Th:value_func}.
% \begin{proof}
% 	Let us denote the $\sigma-$ fields generated by the trajectory $\left\{Q_0,x_0^i,a_0^i,r,x_1^i\ldots x_t^i\right\}$ by $\cF_t$. Since all the random variables in the trajectory till time instant $\tau<t$ are $\cF_t-$measurable, the functions $\Delta_t$ and $F_t$ are also $\cF_t-$measurable which satisfies the measurability condition of lemma~\ref{Lemma:main}. Based on assumptions, it is straightforward to show that the first and the second condition of lemma~\ref{Lemma:main} hold true.
	
% 	Let us now proceed to prove the condition $3$ and $4$ of Lemma~\ref{Lemma:main}. 
% 	We have,
% 	\begin{align}
% 	F_t = R_t +\delta V_{t+1} - Q^\star
% 	\end{align}
% 	$Q^\star$ is the optimal value that corresponds to the \mfe of the game. Let us define an operator $T:\mathcal{V}\to\mathcal{V}$ such that
% 	\begin{align}
% 	TQ_t = \mE\left[R_t + \delta V_t\right]
% 	\end{align}
% 	Now, 
% 	\begin{align}
% 	\left\|\mE\left[F_t\right\vert\cF_t]\right\| &= \left\|\mE\left[R_t+\delta V_t-Q^\star\right]\right\|\\
% 	                                 &= \left\|\mE\left[R_t+\delta V_t-Q^\star + Q_t - Q_t\right]\right\|\nn\\
% 	                                 &\leq \left\|\mE\left[Q_t-Q^\star ]\right]\right\| + \left\|\mE\left[R_t+\delta V_t- Q_t\right]\right\| \nn\\
% 	                                 &\leq \left\|Q_t-Q^\star\right\| + \left\|\mE\left[R_t+\delta V_t- Q_t\right]\right\| \nn\\
% 	                                 &\leq \delta\left\|\Delta_t\right\| + C_t\nn
% 	\end{align}
% 	The third inequality is because of the fact that the policy derived by the fixed point equation forms a contraction mapping. $C_t = \left\|\mE\left[R_t+\delta V_t- Q_t\right]\right\|$ goes to $0$ w.p. $1$ as per the law of large numbers. This proves the third condition for lemma~\ref{Lemma:main}. The 
	
% 	\begin{align}
% 		Var\left\{F_t\vert \cF_t\right\} &= \mE\left[\left(R_t+\delta V_t - Q_t^\star\right)^2\right]\\
% 		 												 &= \mE\left[\left(R_t+\delta V_t - TQ_t^\star\right)^2\right]\\
% 		 												 &= \mE\left[\left(R_t+\delta V_t - \mE\left[R_t + \delta V_t\right]\right)^2\right]\\
% 		 												 &= Var\left\{R_t+\delta V_t\right\}\\
% 		 												 &\leq K\left[1+{\left\|\Delta_t\right\|}^2\right]		 												 
% 	\end{align}

==> STACKELBERG/6Numerical_problems.tex <==

In this section, we consider an example of a repeated Stackelberg security game~\cite{Vasal} to demonstrate the results of our \rl algorithm. We assume a state space $\cX\in\{0,1\}$ and action spaces $\cA^l\in\{0,1\}, \cA^f\in\{0,1\}$ for leader and the follower respectively. The state transition matrix i.e. $\tau\left(x_{t+1}|x_t,a_t\right) = .1$ if $x_t=x_{t+1}$ and $0.9$ otherwise. We assume the discounting factor $\delta = 0.6$. The rewards corresponding to the actions of one player is dependent both the state and the actions of the other player. This is tabulated in~\ref{tab:reward_state0} and~\ref{tab:reward_state1} for state $0$ and state $1$ respectively. 

\figref{fig:Figure_P1_01} and \figref{fig:Figure_P1_11} show the \mpse policies $\tgammatf$ of the follower at different values of the estimated belief state $\pih_t$ for states $x_t=0$ and $x_t=1$ respectively. The plotted graphs are the probabilities with which we choose action $a_t^i =1$.  \figref{fig:Figure_P2_1} show the \mpse policies of the leader pertaining to the probabilities of taking action $a_t^l=1$ given a belief state $\pih_t$. The plots of our algorithm are compared across the true strategy that was obtained by assuming the knowledge of the dynamics of \mdp and then solving the fixed point equation. The strategies estimated using the proposed \rl algorithm coincides with the true optimal establishing the accuracy of our algorithm.
\begin{table}[ht]
	\centering
	\caption{Reward Matrix for $x_t = 0$}
	\begin{tabular}{|cc|c|c|}
		\hline
		&      & Attacker & Attacker\\
		&      & $A1$     & $A2$ \\
		\hline
		Defender  	& $D1$ & $(2,1)$  & $(4,0)$ \\
		\hline          
		Defender    & $D2$ & $(1,0)$  & $(3,2)$ \\
		\hline
	\end{tabular}
	\label{tab:reward_state0}
\end{table}

\begin{table}[ht]
	\centering
	\caption{Reward Matrix for $x_t = 1$}
	\begin{tabular}{|cc|c|c|}
		\hline
		&      & Attacker & Attacker\\
		&      & $A1$     & $A2$ \\
		\hline
		Defender  	& $D1$ & $(2,1)$  & $(4,0)$ \\
		\hline          
		Defender    & $D2$ & $(1,0)$  & $(3,2)$ \\
		\hline
	\end{tabular}
	\label{tab:reward_state1}
\end{table}
\begin{figure}[!htb] %  figure placement: here, top, bottom, or page
	\centering
	\includegraphics[width=.3\textwidth]{Figure_P1_01.pdf} 
	\caption{$\tgamma_t^l(1|0)$: Follower's action given $x_t = 0$ for all belief state under \mpse}
	\label{fig:Figure_P1_01}
\end{figure}
\begin{figure}[!htb] %  figure placement: here, top, bottom, or page
	\centering
	\includegraphics[width=.3\textwidth]{Figure_P1_11.pdf} 
	\caption{$\tgamma_t^f(1|1x)$: Follower's action given $x_t = 1$ for all belief state under \mpse}
	\label{fig:Figure_P1_11}
\end{figure}
\begin{figure}[!htb] %  figure placement: here, top, bottom, or page
	\centering
	\includegraphics[width=.3\textwidth]{Figure_P2_1.pdf} 
	\caption{$\tgamma_t^l(1|0)$: Leader's action corresponding to its \mpse policy}
	\label{fig:Figure_P2_1}
\end{figure}

==> STACKELBERG/7Conclusion.tex <==
\label{sec:concl}
In this paper, we analyzed a stochastic Stackelberg game where there is a leader and a follower. Follower has a private type which evolves in a controlled Markovian fashion, whose statistics are not known to both the players. We proposed a \rl algorithm, based on Expected Sarsa along with particle filters to learn the dynamics of the model by sampling and estimate the $Q_t^f$ and $Q_t^l$ functions that captures the rewards achieved following different policies from a particular state for both the players. Then, using the \mpse algorithm presented in~\cite{Vasal} to converge upon the perfect Stackelberg equilibrium of the game for both the players within a $\epsilon$ margin. 
